A non-intrusive bi-fidelity reduced basis method for time-independent problems

Scientific and engineering problems often involve parametric partial differential equations (PDEs), such as uncertainty quantification, optimizations, and inverse problems. However, solving these PDEs repeatedly can be prohibitively expensive, especially for large-scale complex applications. To address this issue, reduced order modeling (ROM) has emerged as an effective method to reduce computational costs. However, ROM often requires significant modifications to the existing code, which can be time-consuming and complex, particularly for large-scale legacy codes. Non-intrusive methods have gained attention as an alternative approach. However, most existing non-intrusive approaches are purely data-driven and may not respect the underlying physics laws during the online stage, resulting in less accurate approximations of the reduced solution. In this study, we propose a new non-intrusive bi-fidelity reduced basis method for time-independent parametric PDEs. Our algorithm utilizes the discrete operator, solutions, and right-hand sides obtained from the high-fidelity legacy solver. By leveraging a low-fidelity model, we efficiently construct the reduced operator and right-hand side for new parameter values during the online stage. Unlike other non-intrusive ROM methods, we enforce the reduced equation during the online stage. In addition, the non-intrusive nature of our algorithm makes it straightforward and applicable to general nonlinear time-independent problems. We demonstrate its performance through several benchmark examples, including nonlinear and multiscale PDEs.

==> Analysis.tex <==


\section{Numerical examples}
%\textcolor{red}{hardware setting}
In this section, we present numerical results to validate the robustness of our proposed approach for some benchmark examples. We test our algorithm with both linear and nonlinear problems and some of the examples involve the multiscale high-contrast media. The existing reduced basis techniques specialized for (nonlinear) multiscale high-contrast problems are intrusive and mostly require solving a series of local problems in the online stage to construct multiscale problems \cite{efendiev2013generalized, calo2014multiscale, ou2020low}. We check the applicability of our non-intrusive algorithm for this type of problems.
To quantify the accuracy of our method, we compute the following errors. 
\begin{equation}
%e_{L^{rb}} &= \frac{\norm{L_c^{rb}-L_h^{rb}}_2}{\norm{L_h^{rb}}_2}, \\
e_{u,l^2} = \frac{\norm{u_{r}(\mu)  -u_{h}(\mu)}_{l^2}}{\norm{ u_{h}(\mu)}_{l^2}}, \ \ 
%e_{u,H^1} = \frac{\norm{u_{r}(x,\mu)  -u_{h}(x,\mu)}_{H^1(\Omega)}}{\norm{ u_{h}(x,\mu)}_{H^1(\Omega)}}, \label{eq:error1}\\
e_{u,l^2}^l = \frac{\norm{u_{l}(\mu)  -u_{h}(\mu)}_{l^2}}{\norm{ u_{h}(\mu)}_{l^2}}, \ \ 
%e_{u,H^1}^l = \frac{\norm{u_{l}(x,\mu)  -u_{h}(x,\mu)}_{H^1(\Omega)}}{\norm{ u_{h}(x,\mu)}_{H^1(\Omega)}},\label{eq:error2}
\end{equation}
where $u_{r}$ is our reduced solution and
%the coefficient matrix $M_c$ and $M_{ref}$ are computed using coarse and fine operators respectively, and 
 the reference solution $u_h$ represents the full-order FEM solution, and $u_l$ is the solution of the low-fidelity models used for each example. 

Throughout the example sections, we compare our method with another existing bi-fidelity method where the reduced equation is not constructed. The reference bi-fidelity method utilizes the similar strategy in \cite{narayan2014stochastic} using the Cholesky decomposition to select important parameters of low-fidelity solution data. For a new parameter $\mu$, they find the expansion coefficients $c_l(\mu)$ solving least squares problems with low-fidelity solution data. The low-fidelity coefficients $c_l(\mu)$ serve as the expansion coefficients in the approximation of high-fidelity solution at $\mu$.
\beq
u_h(\mu) \approx \sum\limits_{j=1}^{N_{rb}} c_l(\mu) u_h(\mu_j),
\eeq
where $\mu_j$'s are the selected parameters. 
One of the main features in our proposed method is the use of equation information in the online stage, which is not included in the above method. We will often refer to the reference method and our proposed method as `old bi-fidelity method' and `new bi-fidelity method' respectively.
We used MATLAB implementations for both reference and proposed solutions in all examples. All implementations are carried out on a MacBook pro using Apple M1 pro chip with 10-core CPU.

% \textcolor{purple}{can we complete the example section with reference, setup,  of the example and descriptions and interpretation of the results ?}
\subsection{Anisotropic wavespeed simulation}
We consider the following anisotropic wavespeed equation in the domain $\Omega = [-1,1]^2$ introduced in \cite{chen2013reduced}.
\beq
\label{eq:wavespeed}
\begin{split}
-u_{xx}-\mu_1 u_{yy} - \mu_2 u &= -10 \sin(8x(y-1)), \ \  \textrm{in} \ \ \Omega,\\
u &= 0 \ \ \textrm{on} \ \ \partial\Omega,
\end{split}
\eeq
where the parameter domain $D = [0.1,4]\times [0,2]$. Our  full order FEM model has $128\times 128$ fine grids. %To construct a reduced-order model following our algorithm, 
The coarse model by FEM is solved $8\times 8$ grids. We generate $M = 400$ coarse solutions by the coarse solver over the $n_p=400$ equidistant parameters in $\Gamma$. We selected dominant fine solutions at $n_u=21$ of the $400$ parameters to obtain $U_{h,\gamma}$ by QR factorization. Then we perform SVD on $U_{h,\gamma}$ to construct the reduced bases. % in our domain by our QR factorization algorithm,  
We used $3$ parameters in the expansion, i.e., $n_l=3$ in (\ref{eq:LF_expansion}), as we have $\textrm{Rank}(L_{c,\Gamma}) = 3$. %In this example, we do not need to consider the expansion of the right-hand side as in (\ref{eq:LF_expansion}), as our
We remark that the source term does not depend on the parameter in this example. 
Since we have selected $n_u = 21$ and $n_l = 3$ parameters to evaluate the fine solutions and operators,the fine FEM solver was called for  $n_u+n_l = 24$ times in our offline stage to construct $U_{h,\gamma}$ and $L_{h,\gamma}$. 

% \textcolor{red}{what's l? what's the ceterion to choose these numbers?how many fine solver run totally?}
%We are interested in \textcolor{red}{introduce coarse/fine mesh setup} 


Figure \ref{figure:Errors_2D_Wave} shows the error results averaged over $400$ parameters with respect to the number of reduced bases, $N_{rb}$. We observe that both $H^1$, $L^2$ relative errors decrease if the number of reduced bases increases,  the error can reach less than $10^{-3}$ after $9$ reduced bases are used. % which is significantly less than  degrees-of-freedom of our reference full order model, $129\times 129$. 
For a comparison purpose, we plot the error when the coarse model is used solve (\ref{eq:wavespeed}), where  much larger errors can be seen. 
In the figure, we can observe that the old bi-fidelity method performs similarly with our method when small number of reduced bases are used, but the proposed method shows more consistent convergence with number of reduced basis increasing.  
To further demonstrate the approximation quality of the reduced model, 
 Figure \ref{figure:solutions_wave} plots  the  solution computed by the fine solver with the reduced basis solution with $N_{rb} = 12$ reduced bases at $(\mu_1,\mu_2) = (0.305,0.421)$. 
One can see that our reduced solution and truth approximation almost match throughout the domain. Figure \ref{fig:wave_u_coarse} shows that the coarse solver does not provide a good approximation but it captures some important features of the full-order solution. 

Table \ref{tab:wavespeed} shows the computation time with the number of reduced bases, including the offline and online computation time compared to that of full order FEM solve. Once the offline computation is done, the online time is roughly speedup by two orders of magnitude compared to the full order model. It can be seen that  the dominant cost of the online stage  is coarse solve. Note that in the online stage of this example, we only need the coarse operator $L_l(\mu)$ given a parameter $\mu$ from the coarse solver. However we report the computation time for the entire coarse FEM solver (that also provide the coarse solution) as we assume the code for the solver might be locked and we cannot make a partial use of it. 


 
 \begin{figure}[!t]
	\centering
%	\begin{subfigure}{0.45\textwidth}
  \includegraphics[scale =0.45]{figures/l2_romQRBF_colBF_2Dwave.png}
  \caption{Problem (\ref{eq:wavespeed}): The relative errors between the reference fine solution and the reduced solution with different number of reduced basis; The reduced solutions are obtained by our bi-fidelity method and an old bi-fidelity method. The results are compared with the relative errors of the coarse-grid solutions. We report the averaged errors of $400$ results with different parameters. We used $3$ parameters in the expansion of reduced operators ($n_l=3$).}%, and the shaded area is determined by maximum and minimum errors.} %The SVD is performed on full order solutions for $21$ different parameters. We used $3$ parameters in the expansion of operators.}
  \label{figure:Errors_2D_Wave}
 \end{figure}
 

 
\begin{figure}[!htb]
	\centering
	%  \captionsetup{justification=centering}
 	\begin{subfigure}{0.35\textwidth}
  \includegraphics[width=\textwidth]{figures/wave_u_coarse.eps}
  \caption{$u_l$}%with width = 32, depth = 2 $\kappa_{nn} =0.500019
  \label{fig:wave_u_coarse}
\end{subfigure}
 \hspace{-.3in}
   \begin{subfigure}{0.35\textwidth}
  \includegraphics[width=\textwidth]{figures/wave_u_rom_nrb6.eps}
  \caption{$u_{r}$}%with $h=1/100$,\\ $\kappa^*_{FEM} =0.500050879$
  \label{fig:wave_u_rom_rb6}
 \end{subfigure}
\hspace{-.3in}
 	\begin{subfigure}{0.35\textwidth}
  \includegraphics[width=\textwidth]{figures/wave_u_full.eps}
  \caption{$u_h$}%with width = 32, depth = 2 $\kappa_{nn} =0.500019
  \label{fig:wave_u_full}
\end{subfigure}
  \vspace*{-4mm}
 \caption{Problem (\ref{eq:wavespeed}): Solutions obtained by Solutions obtained by coarse model $u_l(x,\mu)$, full model $u_h(x,\mu)$ and reduced model $u_r(x,\mu)$ at $(\mu_1,\mu_2) = (0.305,0.421)$ with the number of reduced basis is $N_{rb}=6$. We used $128\times 128$ fine grid and $8\times 8$ coarse grid. The reduced operator is assembled using $3$ fine operators ($n_l=3$).} %The SVD is performed on $21$ full order solutions for different parameters. We used $3$ parameters in the expansion of operators.}
\label{figure:solutions_wave}
  \vspace*{-3mm}
\end{figure}

% \begin{table}[ht!]
% \centering
% \begin{tabular}{|c||c|c|c|c|c|}
% \hline
% $N_{rb}$&$T_{rb}^{(offline)}$ & $T_{rb}^{(online)}$ &$T_{l}$ & $T_{h}$ & $T_{h}/T_{rb}^{(online)}$  \\
% \hline
% %2 & 0.92182517 & 0.72042995  \\
% 3 & 1.5023s & 3.8320e-4s &2.5469e-4s &4.4722e-2s& 116.7088 \\
% 6 & 1.5054s  & 4.0442e-4s &2.5469e-4s &4.4722e-2s& 110.5851\\
% 9 & 1.5006s  & 4.3267e-4s &2.5469e-4s &4.4722e-2s& 103.3648 \\
% 12 & 1.5014s & 4.6086e-4s &2.5469e-4s &4.4722e-2s& 97.0421\\
% \hline
% \end{tabular}
% \caption{Problem (\ref{eq:wavespeed}): Computation time for offline stage $T_{rb}^{(offline)}$, online stage $T_{rb}^{(online)}$, coarse solver $T_{l}$ and fine solver $T_{h}$ with respect to the number of reduced bases; Computation times $T_{rb}^{(online)}$, $T_{l}$ and $T_{h}$ are averaged over $400$ parameters.}
% \label{tab:wavespeed}
% \end{table}

\begin{table}[ht!]
\centering
\begin{tabular}{|c||c|c|c|c|c|}
\hline
$N_{rb}$&$T_{rb}^{(offline)}$ & $T_{rb}^{(online)}$ &$T_{l}$ & $T_{h}$ & $T_{h}/T_{rb}^{(online)}$  \\
\hline
%2 & 0.92182517 & 0.72042995  \\
3 & 1.4421s & 4.0905e-4s &2.9904e-4s &5.4681e-2s& 133.6780  \\
6 & 1.4565s  & 4.4328e-4s &2.9904e-4s &5.4681e-2s& 123.3554\\
9 & 1.4569s  & 4.7147e-4s &2.9904e-4s &5.4681e-2s& 115.9798 \\
12 & 1.4619s & 5.1501e-4s &2.9904e-4s &5.4681e-2s& 106.1746\\
\hline
\end{tabular}
\caption{Problem (\ref{eq:wavespeed}): Computation time for offline stage $T_{rb}^{(offline)}$, online stage $T_{rb}^{(online)}$, coarse solver $T_{l}$ and fine solver $T_{h}$ with respect to the number of reduced bases; Computation times $T_{rb}^{(online)}$, $T_{l}$ and $T_{h}$ are averaged over $400$ parameters.}
\label{tab:wavespeed}
\end{table}




\clearpage
\subsection{2d nonlinear elliptic equation}
We next consider the following nonlinear elliptic equations defined in $\Omega = [-\frac{\pi}{2},\frac{\pi}{2}]^2$ inspired by the first example in \cite{hesthaven2018non}.
\beq
\label{eq:2dnonlinear}
\begin{split}
-\nabla \cdot [(2+e^{u(x,\mu)}) \nabla u(x,\mu)] = f(x,\mu), \ \  &\textrm{in} \ \ \Omega,
%u(x,\mu) = 0 \ \  &\textrm{on} \ \ \partial\Omega.
\end{split}
\eeq
where  the Dirichlet boundary condition is imposed and the parameters $\mu = 
(\mu_1,\mu_2,\mu_3)$ are chosen from $[1,2]\times[1,2]\times[-0.5,0.5]$. The source term and boundary condition are parameter-dependent and determined so that the exact solution is
\beq
u(x,\mu) = \mu_2 \sin(2+\mu_1 x_1) e^{\mu_3 x_2},
\eeq
where $x = (x_1,x_2)$.
%We note that in this example, the source and boundary condition also depend on the parameters. 

We initially consider $10\times 10\times 10$ equidistant parameters to build reduced model. 
We use our reduced model to solve this problem at the given parameters. For a reference full order model, we use $128\times 128$ FEM grids. Our coarse-mesh FEM uses $10\times 10$ finite elements. The SVD is conducted on the set of full-order solutions that correspond to $20$ parameters ($n_u=20$) selected from the $1000$ equidistant parameters to produce the reduced bases. We use $40$ and $60$ parameters in the expansions of operators and right-hand sides respectively, i.e. $n_l=40$ and $n_f = 60$ (\ref{eq:LF_expansion}). We performed total \textcolor{red}{$n_u+n_l+n_f =120$} fine solve during the offline stage. \textcolor{red}{check epfl paper for their fine solve}


Figure \ref{figure:2dnonlinear} represents the relative errors of our reduced basis method and coarse-grid FEM compared to the corresponding full-order solutions. We can see that the error converges with respect to the number of reduced bases. The relative $L^2$ errors can reach  a level of ${\mathcal O}(10^{-4})$ when  more than $12$ reduced basis are used. % If we directly use our coarse FEM mesh to solve (\ref{eq:2dnonlinear}), we obtain 
In contrast, the coarse model produced inaccurate solutions with relatively large errors as shown in the figure. 
In most of the implementations, our method is better than the reference bi-fidelity method in terms of accuracy due to the use of equation information via reduced equation construction in the online stage. 

Figure \ref{figure:solutions_2DNL} shows the solution plots for full-order model and our reduced-order model with $9$ basis computed at a parameter $(1.05, 1.95,-0.45)$. The two solutions are very close over the entire domain. Table \ref{tab:2dnonlinear2} shows computation time for offline and online stage of our method with different number of reduced bases and computation savings. We achieved a speed-up range of $270-285$.
\textcolor{red}{check how yanlai comments his speedup}


 
 \begin{figure}[!htb]
	\centering
%	\begin{subfigure}{0.45\textwidth}
  \includegraphics[scale =0.45]{figures/l2_romQRBF_colBF_2DNL.png}
  \caption{Problem (\ref{eq:2dnonlinear}): The relative errors between the reference fine solution and the reduced solution with different number of reduced basis; The reduced solutions are obtained by our bi-fidelity method and an old bi-fidelity method. The results are compared with the relative errors of the coarse-grid solutions. We report the averaged errors of $1000$ results with different parameters. We used $40$ and $60$ parameters in the expansion of reduced operators and right-hand sides respectively ($n_l=40$, $n_f=60$).}%, and the shaded area is determined by maximum and minimum errors.}
  \label{figure:2dnonlinear}
 \end{figure}

\begin{figure}[!htb]
	\centering
	%  \captionsetup{justification=centering}
		\begin{subfigure}{0.35\textwidth}
  \includegraphics[width=\textwidth]{figures/2DNL_u_coarse.eps}
  \caption{$u_l$}%with width = 32, depth = 2 $\kappa_{nn} =0.500019
  \label{fig:2DNL_u_coarse}
\end{subfigure}
\hspace{-.3in}
	\begin{subfigure}{0.35\textwidth}
  \includegraphics[width=\textwidth]{figures/2DNL_u_full.eps}
  \caption{$u_h$}%with width = 32, depth = 2 $\kappa_{nn} =0.500019
  \label{fig:2DNL_u_full}
\end{subfigure}
 \hspace{-.3in}
 	  \begin{subfigure}{0.35\textwidth}
  \includegraphics[width=\textwidth]{figures/2DNL_u_rom_rb15.eps}
  \caption{$u_{r}$}%with $h=1/100$,\\ $\kappa^*_{FEM} =0.500050879$
  \label{fig:2DNL_u_rom_rb15}
 \end{subfigure}
  \vspace*{-4mm}
 \caption{Problem (\ref{eq:2dnonlinear}): Solutions obtained by coarse model $u_l(x,\mu)$, full model $u_h(x,\mu)$ and reduced model $u_r(x,\mu)$ at $(\mu_1,\mu_2, \mu_3) = (1.05,1.95,-0.45)$ with the number of reduced basis is $N_{rb}=6$. We used $128\times 128$ fine grid and $10\times 10$ coarse grid. The reduced operator and right-hand side are constructed using $40$ and $60$ parameters respectively. ($n_l=40$, $n_f = 60$).\jrp{in this example, our coarse solution with $10\times 10$ grid looks similar to the truth approximation. We might need to skip the figure.}}
\label{figure:solutions_2DNL}
  \vspace*{-3mm}
\end{figure}


\begin{table}[!htb]
\centering
\begin{tabular}{|c||c|c|c|c|c|}
\hline
$N_{rb}$&$T_{rb}^{(offline)}$ & $T_{rb}^{(online)}$ &$T_{l}$ & $T_{h}$ & $T_{h}/T_{rb}^{(online)}$  \\
\hline
%2 & 0.92182517 & 0.72042995  \\
6 &95.4404s& 2.2581e-3s  & 1.9777e-3s &6.4248e-1s& 284.5224\\
%3 &99.597811s& 0.00225807  &0.00197774 &0.64248096& 117.4702  \\
9 &95.4545s & 2.2669e-3s &1.9777e-3s &6.4248e-1s& 283.4179\\
%6 &99.606684s & 0.00226693 &0.00197774 &0.64248096& 116.9519\\
12 & 95.4675s & 2.3037e-3s &1.9777e-3s &6.4248e-1s& 278.8905\\
%9 & 99.722784s & 0.00230373 &0.00197774 &0.64248096& 116.6760\\
15 &95.4837s  & 2.3466e-3s &1.9777e-3s &6.4248e-1s& 273.7919\\
%12 &99.720519 s  &0.00234661 &0.00197774 &0.64248096& 114.9930 \\
\hline
\end{tabular}
\caption{Problem (\ref{eq:2dnonlinear}): Computation time for offline stage $T_{rb}^{(offline)}$, online stage $T_{rb}^{(online)}$, coarse solver $T_{l}$ and fine solver $T_{h}$ with respect to the number of reduced bases; Computation times $T_{rb}^{(online)}$, $T_{l}$ and $T_{h}$ are averaged over $1000$ parameters.}
\label{tab:2dnonlinear2}
\end{table}
%-------------------------------------------








\clearpage
\subsection{2D elliptic problem with high-contrast coefficient}
Motivated by an example in \cite{ou2020low}, we consider the following elliptic equation with high-contrast permeability coefficient. 
\beq
\label{eq:2dhighcontrast}
\begin{split}
-\div(\kappa(x,\mu) \nabla u(x,\mu)) = f(x), \ \  &\textrm{in} \ \ \Omega,\\
u(x,\mu) = 0 \ \  &\textrm{on} \ \ \partial\Omega.
\end{split}
\end{equation}
The permeability coefficient $\kappa(x,\mu)$ is given by
\beq
\label{eq:kappa_high}
\kappa(x,\mu) = \sum\limits_{i=1}^5  \alpha_i(\mu)\kappa_i(x),
\eeq
where $\kappa_i(x)$ for $i = 1,\dots,4$ is the spatially distributed part of coefficients supported in channels, and the value of $\kappa_5(x)$ is $1$ in the matrix (background) and $0$ in channels. The function $\alpha_i(\mu)$ is defined as follows:
\beq
\label{eq:alpha_mu}
\bsp
\alpha_1(\mu) &= \frac{0.8+1.6 \mu_1^4}{1+\mu_1^4},\\
\alpha_2(\mu) &= 1.1+0.8\sin(\mu_1+\mu_2+\mu_3),\\
\alpha_3(\mu) &= 1.1+0.7\cos(\mu_1^2+\mu_2^2+\mu_3^2),\\
\alpha_4(\mu) &= 1.2 - \frac{0.3\mu_3^2}{1+\mu_2^2 \mu_3^2},\\
\alpha_5(\mu) &= 1,
\end{split}
\eeq
where the parameters $\mu = (\mu_1,\mu_2, \mu_3)$ are taken from the parameter domain $[-1,1]^3$. 
Figure \ref{figure:highcontrast_coeffs} plots the coefficient $\kappa(x,\mu)$ with $3$ different parameters. 
For the source function, we take $f(x) = \sin(\pi x_1) \sin(\pi x_2)$. 

\textcolor{red}{We start with $8\times 8\times 8$ evenly spaced parameters to build our reduced model. We consider the finite element method to solve this problem at given parameters. For full order FEM, we use $128\times 128$ finite elements. We construct the reduced order model using the coarse-grid FEM with $4\times 4$ grids. We select dominant full order solutions at $16$ different parameters (among total $512$ parameters) and perform SVD on them to obtain reduced bases. We use $5$ parameters in the expansion (\ref{eq:LF_expansion}), i.e. $n_l=5$.}

Figure \ref{figure:2dhighcontrast} plots the relative errors for different number of reduced basis $N_{rb}$. The error decays very fast with the number of reduced basis. We can achieve both relative $L^2$ and $H^1$ errors around $10^{-9}$ when we have only $8$ reduced bases. In contrast, the coarse solver with $4\times 4$ meshes cannot resolve the finescale feature of the problem well, therefore results in a larger relative error larger than $10^{-1}$. %Though it can be utilized for the reduced basis construction. 
The proposed method is three orders of magnitude better than the reference old bi-fidelity method according to the error result as the equation information is used in the online stage. 
Figure \ref{figure:solutions_2DHigh} shows the solutions figures obtained by full-order and reduced solves. The reduced order solution is obtained with $4$ bases. The solutions are very close to each other over the entire domain and the corresponding $L^2$ error is around $10^{-5}$. In contrast, the coarse solution in the figure is not close to the fine solution, but it roughly captures some information. 

The computation times for this example can be found in Table \ref{tab:2dhighcontrast}. The computation time for the full-order reference solve is nearly $100$ times that of our online stage. 


\textcolor{red}{how fast msfem can solve this problem?}

\begin{figure}[!htb]
	\centering
	%  \captionsetup{justification=centering}
	\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\textwidth]{figures/kappa1_2DHCMS.eps}
  \caption{$\mu=(1,1,\frac{1}{2})$}%with width = 32, depth = 2 $\kappa_{nn} =0.500019
  \label{fig:kappa1_2DHCMS}
\end{subfigure}
\hspace{-.1in}
  \begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\textwidth]{figures/kappa2_2DHCMS.eps}
  \caption{$\mu=(\frac{1}{2},-\frac{2}{3},-1)$}%with $h=1/100$,\\ $\kappa^*_{FEM} =0.500050879$
  \label{fig:kappa2_2DHCMS}
 \end{subfigure}
 \hspace{-.1in}
  \begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\textwidth]{figures/kappa3_2DHCMS.eps}
  \caption{$\mu=(-\frac{1}{2},\frac{2}{3},-\frac{1}{3})$}%with $h=1/100$,\\ $\kappa^*_{FEM} =0.500050879$
  \label{fig:kappa3_2DHCMS}
 \end{subfigure}
  \vspace*{-4mm}
 \caption{Problem (\ref{eq:2dhighcontrast}): Permeability coefficient $\kappa(x,\mu)$ with three different parameters.}
\label{figure:highcontrast_coeffs}
  \vspace*{-3mm}
\end{figure}

% \begin{figure}[!t]
% 	\centering
% %	\begin{subfigure}{0.45\textwidth}
%   \includegraphics[scale =0.45]{figures/2D_Highcontrast_CErrors_Nrb_fill.png}
%   \caption{Problem (\ref{eq:2dhighcontrast}): The relative errors between the reference fine solution and the reduced solution ($n_l=5$) with number  number of reduced bases compared with the relative errors of the coarse-grid solution. Considering the results with $512$ parameters, the lines represent mean errors, and the shaded area is determined by maximum and minimum errors. }
%   \label{figure:2dhighcontrast}
%  \end{figure}
 
 \begin{figure}[!t]
	\centering
%	\begin{subfigure}{0.45\textwidth}
  \includegraphics[scale =0.45]{figures/l2_romQRBF_colBF_2DHC.png}
  \caption{Problem (\ref{eq:2dhighcontrast}):  The relative errors between the reference fine solution and the reduced solution with different number of reduced basis; The reduced solutions are obtained by our bi-fidelity method and an old bi-fidelity method. The results are compared with the relative errors of the coarse-grid solutions. We report the averaged errors of $512$ results with different parameters. We used $5$ parameters in the expansion of reduced operators ($n_l=5$).}%, and the shaded area is determined by maximum and minimum errors. }
  \label{figure:2dhighcontrast}
 \end{figure}

\begin{figure}[!htb]
	\centering
	%  \captionsetup{justification=centering}
		\begin{subfigure}{0.35\textwidth}
  \includegraphics[width=\textwidth]{figures/2DHigh_u_coarse.eps}
  \caption{$u_l$}%with width = 32, depth = 2 $\kappa_{nn} =0.500019
  \label{fig:2DHigh_u_coarse}
\end{subfigure}
 \hspace{-.3in}
	\begin{subfigure}{0.35\textwidth}
  \includegraphics[width=\textwidth]{figures/2D_High_u_full_nb4.eps}
  \caption{$u_h$}%with width = 32, depth = 2 $\kappa_{nn} =0.500019
  \label{fig:2D_High_u_full_nb4}
\end{subfigure}
\hspace{-.3in}
	  \begin{subfigure}{0.35\textwidth}
  \includegraphics[width=\textwidth]{figures/2D_High_u_rom_nb4.eps}
  \caption{$u_{r}$}%with $h=1/100$,\\ $\kappa^*_{FEM} =0.500050879$
  \label{fig:2D_High_u_rom_nb4}
 \end{subfigure}
  \vspace*{-4mm}
 \caption{Problem (\ref{eq:2dhighcontrast}): Solutions obtained by Solutions obtained by coarse model $u_l(x,\mu)$, full model $u_h(x,\mu)$ and reduced model $u_r(x,\mu)$ at $(\mu_1,\mu_2, \mu_3) = (0.625,-0.625,0,875)$ when the number of reduced basis is $N_{rb}=4$; We used $128\times 128$ fine grid and $8\times 8$ coarse grid. The reduced operator is assembled using $5$ fine operators ($n_l=5$).}
\label{figure:solutions_2DHigh}
  \vspace*{-3mm}
\end{figure}



%---------------------------- without quad
%  \begin{table}[ht!]
% \centering
% \begin{tabular}{|c||c|c|c|c|c|}
% \hline
% $N_{rb}$&$T_{rb}^{(offline)}$ & $T_{rb}^{(online)}$ &$T_{l}$ & $T_{h}$ & $T_{h}/T_{rb}^{(online)}$   \\
% \hline
% %2 & 0.92182517 & 0.72042995  \\
% 2 & 14.5797s & 3.2010e-4s & 1.3367e-4s &3.7323e-2s& 116.5983 \\
% 4 & 14.6082s & 3.3761e-4s &1.3367e-4s& 3.7323e-2s& 110.5510\\
% 6 & 14.6153s & 3.6740e-4s &1.3367e-4s& 3.7323e-2s& 101.5872\\
% 8 & 14.6229s & 3.9753e-4s &1.3367e-4s& 3.7323e-2s& 93.8876\\
% \hline
% \end{tabular}
% \caption{Problem (\ref{eq:2dhighcontrast}): Computation time for offline stage $T_{rb}^{(offline)}$, online stage $T_{rb}^{(online)}$, coarse solver $T_{l}$ and fine solver $T_{h}$ with respect to the number of reduced bases; Computation times $T_{rb}^{(online)}$, $T_{l}$ and $T_{h}$ are averaged over $512$ parameters.}
% \label{tab:2dhighcontrast}
% \end{table}
 \begin{table}[ht!]
\centering
\begin{tabular}{|c||c|c|c|c|c|}
\hline
$N_{rb}$&$T_{rb}^{(offline)}$ & $T_{rb}^{(online)}$ &$T_{l}$ & $T_{h}$ & $T_{h}/T_{rb}^{(online)}$   \\
\hline
%2 & 0.92182517 & 0.72042995  \\
2 & 13.7733s & 3.8753e-4s & 2.0885e-4s &3.7323e-2s& 96.3099 \\
4 & 13.7745s & 3.9741e-4s &2.0885e-4s& 3.7323e-2s& 93.9156\\
6 & 13.7765s & 4.0239e-4s &2.0885e-4s& 3.7323e-2s& 92.7533\\
8 & 13.7771s & 4.1041e-4s &2.0885e-4s& 3.7323e-2s& 90.9408\\
\hline
\end{tabular}
\caption{Problem (\ref{eq:2dhighcontrast}): Computation time for offline stage $T_{rb}^{(offline)}$, online stage $T_{rb}^{(online)}$, coarse solver $T_{l}$ and fine solver $T_{h}$ with respect to the number of reduced bases; Computation times $T_{rb}^{(online)}$, $T_{l}$ and $T_{h}$ are averaged over $512$ parameters.}
\label{tab:2dhighcontrast}
\end{table}
%---------------------------------------


%---------------------------------------
 \textcolor{red}{compare with msfem?}
 

\clearpage
\subsection{2d nonlinear scalar multiscale equation}
\textcolor{red}{reference?}
We have the following nonlinear elliptic multiscale equation in $\Omega = [0,1]^2$.
\beq
\label{eq:2dnlhigh}
- \div \left(\kappa(x,\mu) e^{p(x,\mu)} \nabla p(x,\mu) \right) = 2+\sin(x_1)\cos(x_2)  \, \ \textrm{in} \, \ \Omega\,,
\eeq
The coefficient $\kappa(x,\mu)$ is given by (\ref{eq:kappa_high}) and (\ref{eq:alpha_mu}),
where the parameters $\mu = (\mu_1,\mu_2, \mu_3)$ are taken from the parameter domain $[0,1]^3$. We consider $1000$ evenly spaced parameters to construct $\Gamma$. For the full order problem, we use FEM with $128\times 128$ mesh size and for the coarse FEM solve, we have $4\times 4$ grids. We select dominant full order solutions at $15$ different parameters and perform SVD on them to obtain reduced bases. We use $12$ parameters in the expansion (\ref{eq:LF_expansion}), i.e. $n_l=12$. 

Figure \ref{figure:Errors_2D_NL_HC} represents the errors between the full and reduced order solves with different number of reduced bases. 
 We observe that the relative errors decrease when we use more reduced bases. For all experiments, both relative $L^2$ and $H^1$ errors are less than $10^{-3}$. When our  coarse FEM solver is directly used to solve this problem, we cannot obtain good approximations to the reference solution as seen in this figure. Nevertheless, we can still utilize the coarse solver for the construction of our reduced bases which leads to accurate reduced order solutions. According to the figure, the proposed algorithm has higher accuracy compared to the reference bi-fidelity algorithm as it utilizes the reduced equation in the online stage. 
Figure \ref{figure:solutions_2DNLHigh} plots the solutions obtained by both full-order and reduced solves. The reduced order solution is obtained with $6$ bases. The solutions look very close to each other over the entire domain and the corresponding $L^2$ error is less than $10^{-5}$. The coarse model solution is not a good approximation, but it still captures some features of the full-order model. 

Table \ref{tab:2dnlhigh} shows the computation time for our method compared with that of the reference full-order solve. The speedup range is $620-760$ for this example.


 \begin{figure}[!t]
	\centering
%	\begin{subfigure}{0.45\textwidth}
  \includegraphics[scale =0.45]{figures/l2_romQRBF_colBF_2DNLHC.png}
  \caption{Problem (\ref{eq:2dnlhigh}):The relative errors between the reference fine solution and the reduced solution with different number of reduced basis; The reduced solutions are obtained by our bi-fidelity method and an old bi-fidelity method. The results are compared with the relative errors of the coarse-grid solutions. We report the averaged errors of $1000$ results with different parameters. We used $12$ parameters in the expansion of reduced operators ($n_l=12$).}%, and the shaded area is determined by maximum and minimum errors.}
  \label{figure:Errors_2D_NL_HC}
 \end{figure}
 
 \begin{figure}[!htb]
	\centering
	%  \captionsetup{justification=centering}
		\begin{subfigure}{0.35\textwidth}
  \includegraphics[width=\textwidth]{figures/2DNLHigh_u_coarse.eps}
  \caption{$u_l$}%with width = 32, depth = 2 $\kappa_{nn} =0.500019
  \label{fig:2DNLHigh_u_coarse}
\end{subfigure}
 \hspace{-.3in}
	\begin{subfigure}{0.35\textwidth}
  \includegraphics[width=\textwidth]{figures/2DNLHigh_u_full.eps}
  \caption{$u_h$}%with width = 32, depth = 2 $\kappa_{nn} =0.500019
  \label{fig:2DNLHigh_u_full}
\end{subfigure}
\hspace{-.3in}
	  \begin{subfigure}{0.35\textwidth}
  \includegraphics[width=\textwidth]{figures/2DNLHigh_u_rom_rb6.eps}
  \caption{$u_{r}$}%with $h=1/100$,\\ $\kappa^*_{FEM} =0.500050879$
  \label{fig:2DNLHigh_u_rom_rb6}
 \end{subfigure}
  \vspace*{-4mm}
 \caption{Problem (\ref{eq:2dnlhigh}): Solutions obtained by Solutions obtained by coarse model $u_l(x,\mu)$, full model $u_h(x,\mu)$ and reduced model $u_r(x,\mu)$ at $(\mu_1,\mu_2, \mu_3) = (0.05,0.95,0.05)$ when the number of reduced basis is $N_{rb}=6$; We used $128\times 128$ fine grid and $4\times 4$ coarse grid. The reduced operator is assembled using $12$ fine operators ($n_l=12$) }
\label{figure:solutions_2DNLHigh}
  \vspace*{-3mm}
\end{figure}



% \begin{table}[ht!]
% \centering
% \begin{tabular}{|c||c|c|c|c|c|}
% \hline
% $N_{rb}$&$T_{rb}^{(offline)}$ & $T_{rb}^{(online)}$ &$T_{l}$ & $T_{h}$ & $T_{h}/T_{rb}^{(online)}$   \\
% \hline
% 3 & 36.3844s & 4.4481e-4s &2.7674e-4s &3.0350e-1s& 682.3137 \\
% 6 & 36.4154s & 4.8511e-4s & 2.7674e-4s&3.0350e-1s& 625.6313 \\
% 9 &  36.4122s  & 5.2680e-4s  & 2.7674e-4s&3.0350e-1s& 576.1199 \\
% 12 & 36.4105s  & 5.7034e-4s &2.7674e-4s& 3.0350e-1s& 532.1387 \\
% \hline
% \end{tabular}
% \caption{Problem (\ref{eq:2dnlhigh}): Computation time for offline stage $T_{rb}^{(offline)}$, online stage $T_{rb}^{(online)}$, coarse solver $T_{l}$ and fine solver $T_{h}$ with respect to the number of reduced bases; Computation times $T_{rb}^{(online)}$, $T_{l}$ and $T_{h}$ are averaged over $1000$ parameters.}
% \label{tab:2dnlhigh}
% \end{table}
\begin{table}[ht!]
\centering
\begin{tabular}{|c||c|c|c|c|c|}
\hline
$N_{rb}$&$T_{rb}^{(offline)}$ & $T_{rb}^{(online)}$ &$T_{l}$ & $T_{h}$ & $T_{h}/T_{rb}^{(online)}$   \\
\hline
2 & 32.5945s & 4.0133e-4s &2.7674e-4s &3.0350e-1s& 756.2355 \\
4 & 32.6092s & 4.2712e-4s & 2.7674e-4s&3.0350e-1s& 710.5731 \\
6 &  32.6103s  & 4.4796e-4s  & 2.7674e-4s&3.0350e-1s& 677.5158 \\
8 & 32.6153s  & 4.8371e-4s &2.7674e-4s& 3.0350e-1s& 627.4421 \\
\hline
\end{tabular}
\caption{Problem (\ref{eq:2dnlhigh}): Computation time for offline stage $T_{rb}^{(offline)}$, online stage $T_{rb}^{(online)}$, coarse solver $T_{l}$ and fine solver $T_{h}$ with respect to the number of reduced bases; Computation times $T_{rb}^{(online)}$, $T_{l}$ and $T_{h}$ are averaged over $1000$ parameters.}
\label{tab:2dnlhigh}
\end{table}
% with nx_c = 16: 0.00280930. with nx_c = 8: 0.00084350

%-------------------------------



\clearpage
\subsection{2d nonlinear system of multiscale equations}
Motivated by an example in \cite{mai2022constraint}, we consider the following parameterized coupled steady-state system in the domain $\Omega = [0,1]^2$. 
\beq\label{eq:nex}
\bsp
- \div \left(\frac{\kappa_1(x,\mu)}{1+|p_1(x,\mu)|} \nabla p_1(x,\mu) \right) + \frac{10}{1+|p_1(x,\mu)+p_2(x,\mu)|}(p_1(x,\mu)-p_2(x,\mu)) &= f_1(x) \,,\\
%
- \div \left(\frac{\kappa_2(x,\mu)}{1+|p_2(x,\mu)|} \nabla p_2(x,\mu) \right) + \frac{10}{1+ |p_1(x,\mu)+p_2(x,\mu)|}(p_2(x,\mu)-p_1(x,\mu)) &= f_2(x) \,,
\end{split}
\eeq
where it has zero Dirichlet boundary condition and the parameters $\mu = (\mu_1, \mu_2)$ are chosen from $[0,1]^2$. We have the high-contrast permeability fields $\kappa_1(x,\mu)$ and $\kappa_2(x,\mu)$ defined as
\beq
\bsp
\kappa_1(x,\mu) = \mu_1\kappa_{1,1}(x)+(1-\mu_1)\kappa_{1,2}(x),\\
\kappa_2(x,\mu) = \mu_2\kappa_{2,1}(x)+(1-\mu_2)\kappa_{2,2}(x),
\end{split}
\eeq
where $\kappa_{i,j}(x)$ has the high-contrast features that represent inclusions, channels. This type of coefficients are introduced in \cite{efendiev2013generalized}. We consider $400$ different parameters to construct $\Gamma$. Figure \ref{figure:highcontrast_kappas} depicts the coefficients $\kappa_1$, $\kappa_2$ for different parameters. For the full order model, we used $128\times 128$ FEM grids. For our coarse model, we have $4\times 4$ coarse FEM elements. We select $20$ dominant full-order solutions by the QR factorization and perform SVD on them to obtain reduced bases. We have $n_l=10$ in the expansion (\ref{eq:LF_expansion}). 

We report the relative errors averaged over $400$ parameters. 
Figure \ref{figure:Errors_2D_CPnonlinear} shows the relative errors with different number of reduced bases. We can observe clear convergence of the errors with the number of reduced bases. The figure demonstrates that we achieve inaccurate results if we directly use our coarse FEM grid to solve (\ref{eq:nex}), but we can utilize it to construct our reduced basis and reduced operator to obtain good approximations. We observe that our method outperforms the reference old bi-fidelity method in terms of accuracy due to using equation information to find reduce solution in the online stage. Figure \ref{figure:solutions_2CPDNLHigh} plots the solutions from reference FEM with fine grid and our algorithm using $8$ reduced basis functions. Two solutions are very close to each other in the whole domain. In the figure, the coarse solution vaguely captures some features of the system. 

The computations times are presented in Table \ref{tab:2dnonlinearhighcontrast}. We note that the computation time of coarse runs is dominant in the offline stage. Our online stage is three orders of magnitude faster than the fine solver. 

\begin{figure}[!hbt]
	\centering
	%  \captionsetup{justification=centering}
  	  \begin{subfigure}{0.34\textwidth}
  \includegraphics[width=\textwidth]{figures/k11.eps}
  \caption{$\kappa_1(x,\mu)$, $\mu_1 = 0$}%with $h=1/100$,\\ $\kappa^*_{FEM} =0.500050879$
  \label{fig:k11}
 \end{subfigure}
  \hspace{-.17in}
		\begin{subfigure}{0.34\textwidth}
  \includegraphics[width=\textwidth]{figures/k1.eps}
  \caption{$\kappa_1(x,\mu)$, $\mu_1 = 1/2$}%with width = 32, depth = 2 $\kappa_{nn} =0.500019
  \label{fig:k1}
\end{subfigure}
  \hspace{-.17in}
	\begin{subfigure}{0.34\textwidth}
  \includegraphics[width=\textwidth]{figures/k12.eps}
  \caption{$\kappa_1(x,\mu)$, $\mu_1 = 1$}%with width = 32, depth = 2 $\kappa_{nn} =0.500019
  \label{fig:k12}
\end{subfigure}
  \hspace{-.17in}
  \begin{subfigure}{0.34\textwidth}
  \includegraphics[width=\textwidth]{figures/k21.eps}
  \caption{$\kappa_2(x,\mu)$, $\mu_2 = 0$}
  \label{fig:k21}
 \end{subfigure}
  \hspace{-.17in}
  \begin{subfigure}{0.34\textwidth}
  \includegraphics[width=\textwidth]{figures/k2.eps}
  \caption{$\kappa_2(x,\mu)$, $\mu_2 = 1/2$}%with $h=1/100$,\\ $\kappa^*_{FEM} =0.500050879$
  \label{fig:k2}
 \end{subfigure}
  \hspace{-.17in}
  \begin{subfigure}{0.34\textwidth}
  \includegraphics[width=\textwidth]{figures/k22.eps}
  \caption{$\kappa_2(x,\mu)$, $\mu_2 = 1$}%with $h=1/100$,\\ $\kappa^*_{FEM} =0.500050879$
  \label{fig:k22}
 \end{subfigure}
 \vspace*{-4mm}
 \caption{Problem (\ref{eq:nex}): The coefficients $\kappa_1(x,\mu)$, $\kappa_2(x,\mu)$ with $\mu_i = 0, \ 1/2,\ 1$}
\label{figure:highcontrast_kappas}
 \vspace*{-5mm}
\end{figure}



 
 \begin{figure}[ht!]
	\centering
%	\begin{subfigure}{0.45\textwidth}
  \includegraphics[scale =0.45]{figures/l2_romQRBF_colBF_2DCPNLHC.png}
  \caption{Problem (\ref{eq:nex}): The relative errors between the reference fine solution and the reduced solution with different number of reduced basis; The reduced solutions are obtained by our bi-fidelity method and an old bi-fidelity method. The results are compared with the relative errors of the coarse-grid solutions. We report the averaged errors of $1000$ results with different parameters. We used $10$ parameters in the expansion of reduced operators ($n_l=10$).}%, and the shaded area is determined by maximum and minimum errors..}
  \label{figure:Errors_2D_CPnonlinear}
 \end{figure} 
 
\begin{figure}[!htb]
	\centering
	%  \captionsetup{justification=centering}
	\begin{subfigure}{0.35\textwidth}
  \includegraphics[width=\textwidth]{figures/2DCPNLHigh_u1_coarse.eps}
  \caption{$u_{1,l}$}%with width = 32, depth = 2 $\kappa_{nn} =0.500019
  \label{fig:2DCPNLHigh_u1_coarse}
\end{subfigure}
 \hspace{-.3in}
	\begin{subfigure}{0.35\textwidth}
  \includegraphics[width=\textwidth]{figures/2DCPNLHigh_u1_full.eps}
  \caption{$u_{1,h}$}%with width = 32, depth = 2 $\kappa_{nn} =0.500019
  \label{fig:2DCPNLHigh_u_full}
\end{subfigure}
\hspace{-.3in}
  \begin{subfigure}{0.35\textwidth}
  \includegraphics[width=\textwidth]{figures/2DCPNLHigh_u1_rom_rb8.eps}
  \caption{$u_{1,r}$}%with $h=1/100$,\\ $\kappa^*_{FEM} =0.500050879$
  \label{fig:2DCPNLHigh_u_rom_rb12}
 \end{subfigure}
  \vspace*{-4mm}
 \caption{Problem (\ref{eq:nex}): Solutions obtained by coarse model $u_{1,l}(x,\mu)$, full model $u_{1,h}(x,\mu)$ and reduced model $u_{1,r}(x,\mu)$ at $(\mu_1,\mu_2) = (0.05,0.95)$ when the number of reduced basis is $N_{rb}=8$. We used $128\times 128$ fine grid and $8\times 8$ coarse grid. The reduced operator is assembled using $10$ fine operators ($n_l=10$).}
\label{figure:solutions_2CPDNLHigh}
  \vspace*{-3mm}
\end{figure}
. 


\begin{table}[ht!]
\centering
\begin{tabular}{|c||c|c|c|c|c|}
\hline
$N_{rb}$&$T_{rb}^{(offline)}$ & $T_{rb}^{(online)}$ &$T_{l}$ & $T_{h}$ & $T_{h}/T_{rb}^{(online)}$  \\
\hline
2 & 77.6045s&3.0852e-3s &2.4658e-3s &3.5048s& 1.1361e+3\\
4 & 77.6296s &3.1643e-3s & 2.4658e-3s&3.5048s& 1.1077e+3 \\
6 & 77.6333s  &3.2416e-3s & 2.4658e-3s&3.5048s& 1.0811e+3 \\
8 & 77.6440s &3.3993e-3s & 2.4658e-3s &3.5048s& 1.0311e+3 \\
\hline
\end{tabular}
\caption{Problem (\ref{eq:nex}): Computation time for offline stage $T_{rb}^{(offline)}$, online stage $T_{rb}^{(online)}$, coarse solver $T_{l}$ and fine solver $T_{h}$ with respect to the number of reduced bases; Computation times $T_{rb}^{(online)}$, $T_{l}$ and $T_{h}$ are averaged over $400$ parameters.}
\label{tab:2dnonlinearhighcontrast}
\end{table}
%-----------------------------------------------

\clearpage
 \subsection{Cubic reaction-diffusion equation}
 We have the following reaction-diffusion equation considered in \cite{chen2019l1}.
\beq
 \label{eq:cubic}
 \bsp
-\mu_2\Delta u + u(u-\mu_1)^2 &= f(x) \ \ \textrm{in} \ \ \Omega,\\
u &= 0  \ \ \textrm{on} \ \ \partial \Omega.
 \end{split}
 \eeq
 The parameters $(\mu_1,\mu_2)$ are chosen from $[0.4,5]\times[0.4,2]$.
% The domain $\Omega = [-1,1]^2$ is partitioned into $200\times 200$ finite elements for the reference full-order model. For coarse solve, we use FEM with $10\times 10$ grids. \textcolor{red}{the mesh size is different from yanlai's paper. It is not fair to compare with his results; you may the parameter in table 3 in his paper with the same mesh size $K=200, 400, 800$ for fine mesh.} 
We consider fine solutions at $400$ discrete parameters. The reduced bases are selected using SVD on $28$ dominant fine-grid solutions. The operator for the given parameter is approximated by fine operators computed at $16$ different parameters. 

Figure \ref{figure:Errors_2D_cubic} presents the relative errors. The errors between the direct fine-grid FEM and our reduced order method decrease as we use more reduced bases. We note that the direct FEM solve using coarse grid gives inaccurate solutions but the results show that we successfully constructed the dominant solutions and operators using the coarse mesh.
The figure shows the accuracy of the proposed algorithm is higher than the reference bi-fidelity method without equation construction in the online stage. 
Figure \ref{figure:solutions_cubic} shows the solutions is well recovered by using $12$ reduced bases. 
Table \ref{tab:cubic2} presents the computation time for our offline/online process, coarse solver and the full-order fine-gird FEM solver. The table shows that the online computation is around $600$ times faster than the full-order model computation. 

%  %\begin{figure}[ht!]
%  \begin{figure}[!htb]
% 	\centering
% %	\begin{subfigure}{0.45\textwidth}
%   \includegraphics[scale =0.45]{figures/2D_Cubic_CErrors_Nrb_fill.png}
%   \caption{Problem (\ref{eq:cubic}): The relative errors between the reference fine solution and the reduced solution ($n_l=23$) with number of reduced bases compared with the relative errors of the coarse-grid solution. We report the averaged errors of $1000$ results with different parameters.}
%   \label{figure:Errors_2D_cubic}
%  \end{figure}

  \begin{figure}[!htb]
	\centering
%	\begin{subfigure}{0.45\textwidth}
  \includegraphics[scale =0.45]{figures/l2_romQRBF_colBF_2Dcubic.png}
  \caption{Problem (\ref{eq:cubic}): The relative errors between the reference fine solution and the reduced solution with different number of reduced basis; The reduced solutions are obtained by our bi-fidelity method and an old bi-fidelity method. The results are compared with the relative errors of the coarse-grid solutions. We report the averaged errors of $400$ results with different parameters. We used $16$ parameters in the expansion of reduced operators ($n_l=16$).}
  \label{figure:Errors_2D_cubic}
 \end{figure}

\begin{figure}[!htb]
	\centering
	%  \captionsetup{justification=centering}
 \begin{subfigure}{0.35\textwidth}
  \includegraphics[width=\textwidth]{figures/2DCubic_u_coarse_nrb6.eps}
  \caption{$u_l$}%with width = 32, depth = 2 $\kappa_{nn} =0.500019
  \label{fig:2DCubic_u_coarse}
 \end{subfigure}
 \hspace{-.3in}
	\begin{subfigure}{0.35\textwidth}
  \includegraphics[width=\textwidth]{figures/2DCubic_u_full_nrb6.eps}
  \caption{$u_h$}%with width = 32, depth = 2 $\kappa_{nn} =0.500019
  \label{fig:2DCubic_u_full}
\end{subfigure}
\hspace{-.3in}
	\begin{subfigure}{0.35\textwidth}
  \includegraphics[width=\textwidth]{figures/2DCubic_u_rom_nrb6.eps}
  \caption{$u_{r}$}%with $h=1/100$,\\ $\kappa^*_{FEM} =0.500050879$
  \label{fig:2DCubic_u_rb12}
 \end{subfigure}
  \vspace*{-4mm}
 \caption{Problem (\ref{eq:cubic}): Solutions obtained by coarse model $u_l(x,\mu)$, full model $u_h(x,\mu)$ and reduced model $u_r(x,\mu)$ at $(\mu_1,\mu_2) = (0.515,1.160)$ when the number of reduced basis is $N_{rb}=6$. We used $200\times 200$ fine grid and $10\times 10$ coarse grid. The reduced operator is assembled using $16$ fine operators ($n_l=16$). }
\label{figure:solutions_cubic}
  \vspace*{-3mm}
\end{figure}





%  \begin{table}[ht!]
% \centering
% \begin{tabular}{|c||c|c|c|c|c|}
% \hline
% $N_{rb}$&$T_{rb}^{(offline)}$ & $T_{rb}^{(online)}$ &$T_{c}$ & $T_{h}$ & $T_{fine}/T_{rb}^{(online)}$  \\
% \hline
% %2 & 0.92182517 & 0.72042995  \\
% 3 &148.0280s & 3.0352e-3s  &1.7286e-3s &1.5845s& 522.1000  \\
% 6 &148.0710s   &3.0523e-3s  &1.7286e-3s &1.5845s& 519.1919 \\
% 9 &148.0559s & 3.0622e-3s & 1.7286e-3s&1.5845s& 517.4963\\
% 12 & 148.0804s &3.0679e-3s & 1.7286e-3s &1.5845s& 516.4842\\
% \hline
% \end{tabular}
% \caption{Problem (\ref{eq:cubic}): Computation time for offline stage $T_{rb}^{(offline)}$, online stage $T_{rb}^{(online)}$, coarse solver $T_{c}$ and fine solver $T_{h}$ with respect to the number of reduced bases; Computation times $T_{rb}^{(online)}$, $T_{c}$ and $T_{h}$ are averaged over $400$ parameters.}
% \label{tab:cubic2}
% \end{table}

 \begin{table}[ht!]
\centering
\begin{tabular}{|c||c|c|c|c|c|}
\hline
$N_{rb}$&$T_{rb}^{(offline)}$ & $T_{rb}^{(online)}$ &$T_{c}$ & $T_{h}$ & $T_{fine}/T_{rb}^{(online)}$  \\
\hline
%2 & 0.92182517 & 0.72042995  \\
3 &144.4821s & 2.4035e-3s  &2.1762e-3s &1.5045s& 625.9621  \\
6 &144.5038s   &2.4705e-3s  &2.1762e-3s &1.5045s& 608.9860 \\
9 &144.5128s & 2.4856e-3s & 2.1762e-3s&1.5045s& 605.2864\\
12 & 144.5182s &2.5229e-3s & 2.1762e-3s &1.5045s& 596.3375\\
\hline
\end{tabular}
\caption{Problem (\ref{eq:cubic}): Computation time for offline stage $T_{rb}^{(offline)}$, online stage $T_{rb}^{(online)}$, coarse solver $T_{c}$ and fine solver $T_{h}$ with respect to the number of reduced bases; Computation times $T_{rb}^{(online)}$, $T_{c}$ and $T_{h}$ are averaged over $400$ parameters.}
\label{tab:cubic2}
\end{table}

%-----------------------------------------------------------------------


==> SC.tex <==
\section{Stochastic collocation method}
\label{sec:SC}

One obvious and straightforward way to extend the deterministic AP
schemes to PDE with random inputs is to employ stochastic collocation
method. In stochastic collocation, we first sample the input random
variable $z\in\mathbb{R}^d$, $d\geq 1$. Let $\{z^{(j)}\}_{j=1}^{N_s}$ be the set of samples,
where $N_s$ is the total number of samples, we
then apply a deterministic numerical solver to the underlying
deterministic equations for each fixed sample $z^{(j)}$, for
$j=1,\dots,N_s$, and obtain the solution ensemble $u^{(j)}(x,t) =
u(x,t,z^{(j)})$.
For the hyperbolic and transport equation with diffusive scalings,
this means we need to apply the deterministic AP scheme, with the proper
time relaxation, to each sample simulations. This should a very
straightforward procedure and pose no coding difficulty.

Equipped with the solution ensembles $\{z^{(j)},
u^{(j)}(x,t)\}_{j=1}^{N_s}$, we then, in the post-processing step,
seek to construct an accurate gPC polynomial approximation in the form
of \eqref{gpc_apprx-1}. There exist a variety of ways to construct the
approximating polynomial. For example, one can adopt an interpolation
approach, a regression approach, a discrete projection approach, etc.
For an overview of stochastic collocation methods, see, for example,
\cite{Xiu10}.

Although stochastic collocation is easy to implement in practice, we
remark that it is not desirable in this situation. This is because
although each solution samples are solved via a deterministic AP
scheme, thus guaranteeing their desired diffusive limiting behavior,
there is no guarantee that the gPC expansion $u_N(x,t,z)$ is AP for
any values of $z$. In fact, in most cases, due to the
approximation errors induced by the polynomial reconstruction, it is
almost guaranteed that $u_N(x,t,z)$ will not be AP outside the sample
locations $\{z^{(j)}\}_{j=1}^{N_s}$. The situation becomes more severe
in high dimensional random space with $d\gg 1$. As in this case, the
number of sample $N_s$ becomes large for high-order gPC
approximations. It is then common that one can only afford to
construct a relatively low order gPC approximation. The approximation
errors become much more notable and prevent the solution to be AP for
most values of $z$.

On the other hand, the gPC Galerkin method discussed in the previous
section remains AP for any values of $z$, regardless of the order of
gPC expansion. Therefore, even though the gPC Galerkin method requires
more work in derivation and implementation, it is more desirable in
this case.

We also remark that in some cases one is only interested in the
solution statistics, for example, the mean and standard deviation of
the solution. In this case, the stochastic collocation method is used
as a sampling scheme. The samples $\{z^{(j)}\}$ are chosen from an
integration rule, along with their corresponding weights
$\{w^{(j)}\}$, such that integrals of functions can approximated by
\begin{equation*}
\int f(z)\rho(z) dz \approx \sum_{j=1}^{N_s} f(z^{(j)}) w^{(j)}.
\end{equation*}
For example, in Monte Carlo sampling, $\{z^{(j)}\}$ are randomly sampled with
respect to $\rho(z)$ and $w^{(j)}=1/N_s$. In other deterministic
sampling, $\{z^{(j)}, w^{(j)}\}$ are typically chosen from a
quadrature/cubature rule. Since one is not interested in the solution
$u(x,t,z)$ at any arbitrary location of $z$, the stochastic
collocation can be a more effective way to compute the solution
statistics than the stochastic Galerkin approach.

==> Setup_nonlinear.tex <==

\section{Problem setup}

For ease of presentation, we consider the following nonlinear time-independent parametrized partial differential equations: \textcolor{red}{is this linear pde setting? we should write down the general nonlinear setting}
\jrp{
\beq
\label{eq:main}
{\mathcal L}(u(x,\mu);\mu) = f(x,\mu), \ \  x \in  \Omega \subset \mathbb{R}^n,
\eeq
}
where ${\mathcal L} (\cdot;\mu) $ is the differential operator and some proper boundary conditions are given. For a given physical/uncertain parameter $\mu = (\mu_1, \mu_2, \dots, \mu_d) \in D\subset \mathbb{R}^d$, the solutions to (\ref{eq:main}) are often approximated by solving the corresponding discrete system:
\jrp{
\beq
\label{eq:main_discrete}
L_h(u_h(\mu);\mu) u_h(\mu) = f_h(\mu),
\eeq
}
where $L_h(u_h(\mu);\mu)\in \mathbb{R}^{N_h\times N_h}$ represent the discrete operator and $u_h(\mu)\in\mathbb{R}^{N_h}$ is the approximated  solution. \jrp{Since this is a nonlinear system of equation for $u_h(\mu)$, it is typically solved using an iterative method such as Picard iteration and Newton's method. Also, the number $N_h$ is typically very large to provide a sufficiently accurate approximation to $u(x,\mu)$ in (\ref{eq:main}), therefore solving such a problem with a large $N_h$ is typically computationally expensive, particularly when a large number of high-fidelity solver runs are needed.}  This is particularly evident in applications involving uncertainty quantification, design and optimization, as well as inverse problems. 

% \textcolor{red}{
% \beq
% \label{eq:main_discrete_tmp}
% L_h(u_h^{S-1}(\mu);\mu) u_h^S(\mu) = f_h(\mu),
% \eeq
% }

% \beq
% \label{eq:main_discrete_tmp}
% L_h(u_h^{S-1}(\mu);\mu) \approx \sum\limits_{j=1}^{n_L} L_h(u_h^{S-1}(\mu^L_j);\mu^L_j) \, a_h^{(j)}(\mu), \
% \eeq

% The parameters $\mu$ are from \textcolor{red}{${\mathcal D}_\infty$}, a sample space continuous with respect to $\mu$. 
Our goal is to efficiently approximate the solutions of the partial differential equations at a given parameter $\mu$.  The traditional projection-based reduced models make the assumption that the truth solution $u_h(\mu)$ lives in a low-dimensional  manifold, which can be approximated by a reduced approximation space with a dimension $N_{rb}$ much smaller than $N_h$. 
% The solutions at the parameters outside ${\mathcal D}$ are approximated using interpolation. We assume that every point in ${\mathcal D}_\infty$ is sufficiently close to one of the proxies in ${\mathcal D}$.
%The traditional projection-based reduced models typically
% first construct an orthogonal basis matrix $Q \in \mathbb{R}^{N_h\times N_{rb}}$ by \textcolor{red}{by POD or error indicator?}.%, where $N_{rb} \ll N_h$, whose columns form a basis for a reduced model whose solution is $u_{rb}(\mu) \in \mathbb{R}^{N_{rb}}$. 
 Then the solution $u_h(\mu)$ to (\ref{eq:main_discrete}) is approximated by the reduced solution as follows:
 \beq
 \label{eq:reconstructed}
u_h(\mu) \approx u_r(\mu) = Q u_{rb}(\mu),
 \eeq
where  $u_{rb}(\mu)\in \mathbb{R}^{N_{rb}}$ is the orthogonal reduced coefficient vector and $Q \in \mathbb{R}^{N_h\times N_{rb}}$ is the reduced basis that span the reduced approximation space.
 %\textcolor{red}{something is missing here. also need to mention the challenge here for nonlinear problems and intrusiveness, which are the motivations}
By Galerkin projection on the problem (\ref{eq:main}) on the reduced approximation space, we can get the following reduced system:
\jrp{
\beq
\label{eq:reduced}
L_{rb}(u_{rb}(\mu);\mu) u_{rb}(\mu) = f_{rb}(\mu),
\eeq
}
where  the reduced operator $L_{rb}(u_{rb}(\mu);\mu)  \in \mathbb{R}^{N_{rb}\times N_{rb}}$ and the reduced right-hand side $f_{rb}(\mu) \in \mathbb{R}^{N_{rb}}$ are given as follows:
\jrp{
\beq
\label{eq:reduced2-operator}
L_{rb}(u_{rb}(\mu);\mu) = Q^T L_h(Q u_{rb}(\mu);\mu)Q, \quad f_{rb}(\mu) = Q^T f_h(\mu),
\eeq
}
\jrp{For linear problems, the reduced operator $L_{rb}(\mu) = Q^T L_h(\mu)Q$ does not depend on the solution $u_h(\mu)$}, therefore the reduced system (\ref{eq:reduced}) can be solved  efficiently thanks to the reduced dimension $N_{rb} \ll N_h$ for $u_{rb}(\mu)$. 
% We note that $Q^TL_h(\mu)Q$ is in $ \mathbb{R}^{N_{rb}\times N_{rb}}$, thus computation of (\ref{eq:reduced}) is much less expansive than that of the original problem (\ref{eq:main}). 

\textcolor{blue}{ 
Nonetheless, for general nonlinear PDEs, the assembly of the reduced matrix $L_{rb}(u_h(\mu);\mu)$ at the online stage depends on the dimension of the high-fidelity solutions $u_h(\mu)$. Therefore the computational complexity of \eqref{eq:reduced} remains dependent on the dimension of the high-fidelity model, $N_h$.  %For more efficient solve, 
To further improve the efficiency, EIM and its variants are usually needed \cite{barrault2004empirical,chaturantabut2010nonlinear}, where one often needs to  make major modifications to the source code,  %to use or recover the decomposition of $L_h(\mu)$ into the sum of the matrices independent of the parameter that can be pre-computed in offline stage. 
which can be time-consuming and sophisticated, particularly for large-scale complex applications.}% or not possible when the source code of the full-order  model is not accessible. }

To address this challenge, we develop a non-intrusive reduced-order model, particularly to efficiently construct the reduced operator \jrp{$L_{rb}(u_{rb}(\mu);\mu)$} during the online stage in this work. % and the projected right-hand side $Q^T F_h(\mu)$.
% \textcolor{red}{For simplicity, we abuse the notation and denote the nonlinear operators in the same way as the linear counterpart, i.e., we have
% \beq
% L_h(\mu) := L_{h}(u_{h}(\mu);\mu), \ L_{rb}(\mu) := L_{rb}(u_{rb}(\mu);\mu)
% \eeq
% for nonlinear problems. \jrp{may be some other simplified notation}}
We assume we  can access the solutions, assembly operator matrices, and the right-hand side of our model from the existing legacy solver.  We further  assume that  for  any given parameter $\mu \in {\mathcal D}$,  the high-fidelity model operator $L_h(u_h(\mu);\mu) \in \mathbb{R}^{N_h\times N_h}$, and right-hand side $f_h(\mu) \in \mathbb{R}^{N_h}$ can be well approximated by a linear combination of the high-fidelity operators/right-hand side, respectively
% we approximate the full-order model operator %$L_h(\mu) \in \mathbb{R}^{N_h\times N_h}$, and righ-hand side $f_h(\mu) \in \mathbb{R}^{N_h}$ by
\jrp{
\beq
\label{eq:LF_expansion}
L_h(u_h(\mu);\mu) \approx \sum\limits_{j=1}^{n_L} L_h(u_h(\mu^L_j);\mu^L_j) \, a_h^{(j)}(\mu), \ 
f_h(\mu) \approx \sum\limits_{j=1}^{n_f} f_h(\mu^f_j) \, b_h^{(j)}(\mu),
\eeq
}
by properly chosen parameter points  $\{\mu^L_j \in {\mathcal D}, j=1, \hdots,n_L\}$ and  $\{\mu^f_j \in {\mathcal D}, j=1, \hdots,n_f\}$.  The expansion coefficients $a_h^{(j)}(\mu)$ and $b_h^{(j)}(\mu)$ need to be approximated.

In this case, reduced operators $L_{rb}(u_{rb};\mu)$ and reduced right-hand side $f_{rb}(\mu) $ can be approximated as follows:
\jrp{
\beq
\begin{split}
\label{eq:QLF_expansion}
L_{rb}(u_{rb};\mu) &= Q^T L_h(Q u_{rb};\mu) Q \approx Q^T L_h(u_h;\mu) Q \approx \sum\limits_{j=1}^{n_L} [Q^T L_h(u_h;\mu^L_j) Q ]\, a_h^{(j)}(\mu) ,\\
%:= \sum\limits_{j=1}^{n_L} L_{rb}(u_{rb}(\mu);\mu^L_j) \, a_h^{(j)}(\mu) , \\ 
f_{rb}(\mu) &= Q^T f_h(\mu) \approx \sum\limits_{j=1}^{n_f} [Q^T f_h(\mu^f_j)] \, b_h^{(j)}(\mu), 
%:= \sum\limits_{j=1}^{n_f} f_{rb}(\mu^f_j) \, b_h^{(j)}(\mu),
\end{split}
\eeq
%where that the matrices $L_{rb}(\mu^L_j)$ and vectors $f_{rb}(\mu^f_j)$ are independent of the parameter $\mu$, 
where that the matrices $Q^T L_h(u_h;\mu^L_j) Q $ and vectors $Q^T f_h(\mu^f_j)$ are independent of the parameter $\mu$, 
thus can be precomputed during the offline stage.}
As a result, if the expansion coefficients $a_h^{(j)}(\mu)$ and $b_h^{(j)}(\mu)$ can be efficiently approximated during the online stage, the reduced system can be well assembled with reasonable computation cost. 
In \cite{etter2023coarse}, the authors suggest an efficient way to recover the expansion coefficients $a_h^{(j)}(\mu)$ of the operators based on the single fidelity solver.
\jrp{They randomly subsample the rows of the high-fidelity operators to reduce the dimension of the least square problems of finding the expansion coefficients $a_h^{(j)}(\mu)$. However, the randomness involved in the strategy can potentially impede their reconstruction performance.} \textcolor{red}{be more explicitly}
Motivated by their work, we propose a bi-fidelity framework to  efficiently approximate high-fidelity coefficients $a_h^{(j)}(\mu)$ and $b_h^{(j)}(\mu)$ to construct the reduced model in the online stage.
In the next section, we shall discuss our approach to constructing and solving the reduced system \eqref{eq:QLF_expansion}. %$L_{rb}(\mu)$ and the right-hand side $f_{rb}(\mu))$ via (\ref{eq:QLF_expansion}). 

% \beq
% {\mathbb L}(\mu) u_\mu(x) = f(\mu,x), \ \  x\in\Omega \subset \mathbb{R}^n,
% \eeq
% (\jrp{some connection})
% We discretize the above equations using finite element method with $n$ 
% \beq
% \bf{K}(\mu) \bf{U}(\mu) = \bf{F}(\mu),
% \eeq
% where 


\section{Bi-fidelity reduced-based methods}
%\textcolor{blue}{In reduce order modeling, directly constructing the reduced operator and right-hand side  in (\ref{eq:QLF_expansion}) may require many of the high-fidelity  runs (\ref{eq:main_discrete}) with a large set of different parameters to access the high-fidelity information online. This is computationally  expensive to reduce the cost. By assuming that the low-fidelity solutions and operators can capture the essential behaviors and general trends of the high-fidelity solution and operator, respectively, in the parameter space, we can con 
%We employ a bi-fidelity method to utilize both coarse (low-fidelity) and fine (high-fidelity) model in the offline algorithm.} \textcolor{red}{need to rework} %In our algorithm, we would like to replace many full-order solves with coarse solves to significantly reduce the total number of full-order simulations in the offline stage. } 


To set up the stage for the discussion later on, we assume a low-fidelity model corresponding to the high-fidelity (fine-mesh) model (\ref{eq:main}) is available: 
\jrp{
\beq
\label{eq:coarse_main}
L_l(u_l(\mu);\mu) u_l(\mu) = f_l(\mu),
\eeq
where $L_l(u_l(\mu);\mu) \in \mathbb{R}^{N_l \times N_l}$, $u_l(\mu)$, $f_l(\mu) \in \mathbb{R}^{N_l}$ for $N_l \ll N_h$.} 
%We again use the simplified notation $L_l(\mu) := L_l(u_l(\mu);\mu)$ for nonlinear low-fidelity operators.}
The low-fidelity model can be solved much faster than the full-order model due to less number of degrees of freedom.  Although the coarse model is less accurate, %the accuracy of (\ref{eq:coarse_main}) is less than the hi-fidelity model (\ref{eq:main_discrete}) 
the low-fidelity functions $u_l(\mu)$, $L_l(u_l(\mu);\mu)$ and $f_l(\mu)$ can capture some important features of corresponding high-fidelity functions $u_h(\mu)$, $L_h(u_h(\mu);\mu)$ and $f_h(\mu)$ respectively.
%Compared to the high-fidelity model (\ref{eq:main_discrete}), the simulation of (\ref{eq:coarse_main}) is much faster but yields  
\textcolor{red}{For simplicity, we abuse the notation and denote the nonlinear operators in the same way as the linear counterpart, i.e., we have
\beq
L_h(\mu) := L_{h}(u_{h}(\mu);\mu), \ L_l(\mu) := L_{l}(u_{l}(\mu);\mu), \ L_{rb}(\mu) := L_{rb}(u_{rb}(\mu);\mu)
\eeq
for nonlinear problems. \jrp{may be some other simplified notation}}

For a parameter set $\gamma = \{\mu_1, \mu_2, \dots, \mu_{j}\}$, we denote snapshot matrices of low-fidelity solutions, operators, and the right-hand sides evaluated at the points in $\gamma$ as 
\beq
\label{low-snapshots}
\begin{split}
&{\mathcal U}_{l}(\gamma) = [u_l(\mu_1)\ \ u_l(\mu_2)\ \ \dots \ \ u_l(\mu_{j})],\\
&{\mathcal L}_{l}(\gamma) = [\vec{L}_l(\mu_1)\ \ \vec{L}_l(\mu_2)\ \ \dots \ \ \vec{L}_l(\mu_{j})], \\
&{\mathcal F}_{l}(\gamma) = [f_l(\mu_1)\ \ f_l(\mu_2) \ \ \dots \ \ f_l(\mu_{j})],
\end{split}
\eeq
where $\vec{L}$ means the vectorized operators. For example, $\vec{L}_l(\mu_i)$ is a vector of size $N_l^2 \times 1$ containing all entries of the matrix $L_l(\mu_i)\in \mathbb{R}^{N_l \times N_l}$. But in this work, we only consider the nonzero entries of the matrices $L_l(\mu_i)$ to generate $\vec{L}_l(\mu_i)$ for both computational and memory efficiency as the matrix is typically sparse. As a result, the dimension of the vector $\vec{L}_l(\mu_i)$ is ${\mathcal O}(N_l)$, corresponding to the number of nonzero entries of $L_l(\mu_i)$.

Similarly, the snapshot matrices for the full-order solutions can be denoted accordingly.
\beq
\label{high-snapshots}
\begin{split}
& {\mathcal U}_{h}(\gamma) = [u_h(\mu_1)\ \ u_h(\mu_2)\ \ \dots\ \ u_h(\mu_{j})],\\
& {\mathcal L}_{h}(\gamma) = [\vec{L}_h(\mu_1)\ \ \vec{L}_h(\mu_2)\ \ \dots\ \ \vec{L}_h(\mu_{j})], \\
&{\mathcal F}_{h}(\gamma) = [f_h(\mu_1)\ \ f_h(\mu_2)\ \ \dots \ \ f_h(\mu_{j})],
\end{split}
\eeq
 The dimension of the vector $\vec{L}_h(\mu_i)$ is ${\mathcal O}(N_h)$, when the operator is sparse.
In this work, we shall leverage both low-fidelity and high-fidelity models to construct the reduced system efficiently.
%$Q$ and the reduced operator $L_{rb}(\mu)$ and the right-hand side $f_{rb}(\mu)$. We first outline the algorithm
Consider a set of parameters $\Gamma = \{\mu_1, \mu_2, \dots,\mu_{n_p}\}$ dense enough in the parameter domain $D$. \\
{\bf Offline stage}:
\begin{enumerate}
\item Low-fidelity runs
\begin{itemize}
%\item[$-$] 
\item[$-$] Perform low-fidelity simulations at all parameters in $\Gamma$ to obtain ${\mathcal U}_{l}(\Gamma)$, ${\mathcal L}_{l}(\Gamma)$, and ${\mathcal F}_{l}(\Gamma)$ in \eqref{low-snapshots}. 
\item[$-$] Select important parameters from $\Gamma$ to construct $\gamma_u = \{\mu^u_1,\mu^u_2, \dots, \mu^u_{N_{rb}}\}$,  $\gamma_L = \{\mu^L_1,\mu^L_2, \dots, \mu^L_{n_L}\}$, $\gamma_f = \{\mu^f_1,\mu^f_2, \dots, \mu^f_{n_f}\}$ in \eqref{eq:LF_expansion} 
\end{itemize}
\item High-fidelity runs
\begin{itemize}
\item[$-$] Perform high-fidelity simulations at the selected parameter set in $\gamma_u$, $\gamma_L$, and $\gamma_f$ to construct ${\mathcal U}_{h}(\gamma_u)$, ${\mathcal L}_{h}(\gamma_L)$, and ${\mathcal F}_{h}(\gamma_f)$  in \eqref{high-snapshots}. %(The subscript of $\gamma$ will be omitted for matrix notations for simplicity, e.g., ${\mathcal U}_{h}(\gamma_u) = {\mathcal U}_{h}(\gamma)$ )
\end{itemize}
\item Reduced basis construction
\begin{itemize}
\item[$-$]% Perform singular value decomposition to build 
 Construct the reduced basis $Q$ using high-fidelity snapshots matrix ${\mathcal U}_{h}(\gamma_u)$.
\item[$-$] \textcolor{red}{Compute the basis for reduced order operator and reduced 
 right-hand side: $Q^T L_h(\mu^L) Q$ and $Q^T f_{h}(\mu^f)$ in \eqref{eq:QLF_expansion} for all $\mu^L \in \gamma_L$, $\mu^f \in \gamma_f$}
\end{itemize}
{\bf Online stage}:
\item For a given parameter $\mu$, run the corresponding low-fidelity solver to find the expansion coefficients $a_l(\mu)$ and $b_l(\mu)$.
%Low-fidelity least squares problems
%\begin{itemize}
%\item[$-$] Compute ${\mathcal L}_{l}(\gamma)^T {\mathcal L}_{l}(\gamma)$ and $F_{l}(\gamma)^T F_{l}(\gamma)$
%\item[$-$] Compute $\vec{L}_l(\mu)$ for given parameter $\mu$ using low-fidelity solver
%\item[$-$] Find the expansion coefficients $a_l(\mu)$ and $b_l(\mu)$ by least squares problems
%\beq
%{\mathcal L}_{l}(\gamma)^T {\mathcal L}_{l}(\gamma) a_l(\mu) = {\mathcal L}_{l}(\gamma) ^T\vec{L}_l(\mu), \  
%F_{l}(\gamma)^T F_{l}(\gamma) b_l(\mu) = F_{l}(\gamma)^T f_l(\mu).
%\eeq
%\end{itemize}
\item Construct and solve reduced problems
\begin{itemize}
\item[$-$] Assemble the reduced operators and reduced right-hand sides by \eqref{eq:QLF_expansion}
\item[$-$] Solve the reduced system \eqref{eq:reduced}.
%\beq
% \label{eq:QLF_expansion}
%L_{rb}(\mu) \approx \sum\limits_{j=1}^{n_L} L_{rb}(\mu^L_j)\, a_l^{(j)}(\mu), \ 
%f_{rb}(\mu) \approx %\sum\limits_{j=1}^{n_F} f_{rb}(\mu^F_j) \, b_l^{(j)}(\mu),
%\eeq
\end{itemize}
\end{enumerate}
The schematic description of our algorithm is presented in Figure \ref{fig:flowchart}.  We shall explain the details of each building block of the proposed method.
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/ROM_SCHEME_V3.png}
    \caption{Flowchart of the proposed reduced method.}
    \label{fig:flowchart}
\end{figure}

% \textcolor{red}{might be a good idea to list the pesduo code to demonstrate the whole algorithm}

%\subsection{Offline algorithm}
\subsection{Point Selection and Reduced basis construction (Offline)}
We first choose a candidate set of parameters $\Gamma = \{\mu_1, \mu_2, \dots,\mu_{n_p}\} \subset D$ and assume  $\Gamma$ is large enough to represent  the parameter space. %that every parameter $\mu \in D$ is sufficiently close to one of the parameters in $\Gamma$. We consider but do not compute 
We consider the following matrix in $\mathbb{R}^{N_h\times n_p}$ of full order solutions at parameters in $\Gamma$.
\beq
\label{eq:S}
{\mathcal U}_{h}(\Gamma) = [u_h(\mu_1) \ \ u_h(\mu_2) \ \ \dots \ \ u_h(\mu_{n_p})]
\eeq
%To compute allWe want to select important columns of ${\mathcal U}_{h}(\Gamma)$ that will contribute to constructing a 
To construct the projection-based  reduced basis  $Q \in \mathbb{R}^{N_h\times N_{rb}}$, one typically performs $n_p$ high-fidelity simulations to collect all solution snapshots and perform Gram-Schmidt process to extract the reduced basis set. However, the computation of the high-fidelity solutions $u_h(\mu_i)$ at many different parameters $\mu_i$, $i = 1,\dots, n_p$ is very expensive. To reduce the number of high-fidelity samples, we assume the coarse-model solutions can capture the main characteristics of the high-fidelity model in the parameter space.% such that %that the selected parameters $\{\mu^u_1,\mu^u_2, \dots, \mu^u_{n_u}\}$ using $U_{l,\Gamma}$ correspond to important columns in $U_{h,\Gamma}$
%it can be used to guide the selection of important parameter points.  
This idea is widely used in the multi-fidelity literature \cite{zhu2014computational,zhu2017multi,etter2023coarse}. We refer the interested readers for more details in \cite{etter2023coarse}.

Specially, we    
% \beq
% \label{eq:S}
% S = [U_h(\mu_1) \ \ U_h(\mu_2) \ \ \dots \ \ U_h(\mu_p)]
% \eeq
perform the low-fidelity simulations for (\ref{eq:coarse_main}) on 
 the candidate set $\Gamma$  to collect the following $N_l\times n_p$ snapshot matrix of the coarse solutions:
\beq
\label{eq:S_c}
{\mathcal U}_{l}(\Gamma) = [u_l(\mu_1) \ \ u_l(\mu_2) \ \ \dots \ \ u_l(\mu_{n_p})] 
\eeq
To select important parameter points, we perform pivoted Cholesky factorization on ${\mathcal U}_{l}(\Gamma)$.
This procedure provides a permutation of the matrix ${\mathcal U}_{l}(\Gamma)$. We select the columns corresponding to $N_{rb}$ largest diagonal entries of the matrix $R$, and choose the $N_{rb}$ parameters associated with the selected important columns, where $N_{rb}$ represents the dimension of reduced basis. We refer to the selected parameters as $\gamma_u = \{\mu^u_1,\mu^u_2, \dots, \mu^u_{N_{rb}}\} \subset \Gamma$. %\textcolor{red}{can we replace the subindex s to be r so that it can be consistent with ROM literature}
%\textbf{Step 2: Construct reduced basis.}
To construct the reduced basis for the fine mesh solutions,
we run the fine-mesh solver to obtain the high-fidelity solutions (\ref{eq:main}) {\it only} for each point in $\gamma_u$. We  denote the snapshot matrix as follows:
\beq
\label{eq:S_hat}
{\mathcal U}_{h}(\gamma) = [u_h(\mu^u_1) \ \ u_h(\mu^u_2) \ \ \dots \ \ u_h(\mu^u_{N_{rb}})],
\eeq
where ${\mathcal U}_{h}(\gamma_u)$ is   $N_h \times N_{rb}$ and the columns represent important solutions in ${\mathcal U}_{h}(\Gamma)$. 
To form the orthonormal reduced bases, we then perform Gram-Schmidt orthogonalization on ${\mathcal U}_{h}(\gamma_u)$ to obtain the reduced basis set $Q$. The detailed algorithm of this section is presented in Algorithm $1$.

\subsection{Constructing the reduced operator and right-hand side (Offline)}

{\bf Construct the reduced operator}. To select the important points for the reduced operator $L_h(\mu)$ in \eqref{eq:LF_expansion}, 
we consider the following snapshot matrix for the  fine mesh operator $L_h$ whose columns are the vectorized full operators $L_h(\mu)$ in for candidate set $\Gamma$ in the parameter space.
\beq
\label{eq:L}
{\mathcal L}_{h}(\Gamma) = [\vec{L}_h(\mu_1) \ \ \vec{L}_h(\mu_2) \ \ \dots \ \ \vec{L}_h(\mu_{n_p})]
\eeq
%We would like to find the dominant columns of 
if ${\mathcal L}_{h}(\Gamma)$ is available, we can perform pivoted Cholesky decomposition on it to select the important columns.  However, this requires a large number of high-fidelity runs to collect the snapshot matrix. By the same argument used to select important points for $u_h(\mu)$ in the previous section, we assume the coarse-model operator can capture the main characteristics of the high-fidelity operator in the parameter space. Based on this assumption, we construct the corresponding snapshot matrices of operators on a coarse mesh for the candidate set $\Gamma$:
\beq
\label{eq:L_c}
{\mathcal L}_{l}(\Gamma) = [\vec{L}_l(\mu_1) \ \ \vec{L}_l(\mu_2) \ \ \dots \ \ \vec{L}_l(\mu_{n_p})]
\eeq
Note that these matrices ${\mathcal L}_{l}(\Gamma)$ have already been assembled when we build the snapshot matrix ${\mathcal U}_{l}(\Gamma)$ in the previous section. 
We then apply pivoted Cholesky decomposition to ${\mathcal L}_{l}(\Gamma)$. The first $n_L$ elements of the permutation vector give the most important parameters for the operator $L$. We denote the selected parameters as 
\beq
\gamma_L = \{\mu^L_1, \mu^L_2, \dots , \mu^L_{n_L} \} \subset \Gamma.
\eeq
We then perform high-fidelity simulations for each point in $\gamma_L$ to compute the corresponding high-fidelity operators $\{ L_h(\mu^L_i) \ | \ \mu^L_i \in \gamma_L\}$. Then we project them onto the reduced approximation space spanned by the solution reduced basis set $Q$ and construct the reduced basis set $\{ Q^T L_h(\mu^L_i) Q \ | \ \mu^L_i \in \gamma_L \}$ for the reduced operator in (\ref{eq:QLF_expansion}).
During the online stage, the above reduced matrices will be used in the expansion (\ref{eq:QLF_expansion}) of the reduced operator $L_{rb}(\mu)$ at the given parameter $\mu$. 

\textcolor{blue}{
\begin{remark}
Note that all fine and coarse operators can be stored in a sparse format. The actual dimensions of the operator matrices $L_h(\mu)$, $L_l(\mu)$ at each parameter $\mu$ are equal to the number of nonzero entries of them. In many applications, the operator matrices are extremely sparse, and the number of nonzero entries of $L_h(\mu)$, $L_l(\mu)$ are ${\mathcal O}(N_h)$, ${\mathcal O}(N_l)$ respectively. We remark that to generate the vectorized operators $\vec{L}_h(\mu)$ and $\vec{L}_l(\mu)$, we only use the nonzero entries of the operator matrices $L_h(\mu)$ and $L_l(\mu)$. Thus, the dimensions of $\vec{L}_h(\mu)$ and $\vec{L}_l(\mu)$ are ${\mathcal O}(N_h)$, ${\mathcal O}(N_l)$ respectively.
\end{remark}\\
}
\jrp{
%RB literature https://arxiv.org/pdf/2101.05902.pdf
\begin{remark}
Nonlinear problems, where the operators depend on the solution, are typically handled by some iteration methods, e.g., Picard, or Newton's iteration method.  
For example, for our high- and low-fidelity nonlinear models, the iteration methods converge to the numerical solution $u_h(\mu)$ and $u_l(\mu)$ respectively with some convergence criterion. Then correspondingly, the high- and low-fidelity operators converge to $L_h(\mu) := L_h(u_h(\mu);\mu)$ and $L_l(\mu) := L_l(u_l(\mu);\mu)$ throughout the iteration procedures. Notably, our algorithm only utilizes the limit solutions and operators (not the entire sequence of them) from the legacy solver for nonlinear problems. 
\end{remark}
}


%\textbf{Step 3 (Offline): 
{\bf Construct reduced right-hand side}.
%Similar to the point selection for the operator $L_h$,  
 To select the important points for the reduced right-hand side  in \eqref{eq:LF_expansion}, we denote  the following right-hand side snapshot matrix in $\mathbb{R}^{N_h\times n_p}$ as follows:
\beq
\label{eq:F}
{\mathcal F}_{h}(\Gamma) = [f_h(\mu_1) \ \ f_h(\mu_2) \ \ \dots \ \ f_h(\mu_{n_p})]
\eeq
Similarly, we denote the following matrix in $\mathbb{R}^{N_l\times n_p}$ of coarse right-hand sides instead of (\ref{eq:F}). 
\beq
\label{eq:Fc}
{\mathcal F}_{l}(\Gamma) = [f_l(\mu_1) \ \ f_l(\mu_2) \ \ \dots \ \ f_l(\mu_{n_p})]
\eeq

By the same argument for point selection for constructing the reduced operator, we shall select important points informed coarse mesh snapshot matrix ${\mathcal F}_{l}(\Gamma)$, which are already available as they were generated when we obtain ${\mathcal U}_{l}(\Gamma)$ using the coarse solver. We then use pivoted Cholesky decomposition on ${\mathcal F}_{l}(\Gamma)$ to find the corresponding $n_f$ dominant columns. Then we select the parameters corresponding to those columns and denote them by $\gamma_f =  \{\mu^f_1, \mu^f_2, \dots, \mu^f_{n_f} \} \subset \Gamma$.  
% \beq
% \label{eq:Fhhat}
% F_{h,\gamma} = [f_h(\mu^f_1) \ \ f_h(\mu^f_2) \ \ \dots \ \ f_h(\mu^f_{n_f})]
% \eeq
We compute the reduced basis $\{Q^T f_h(\mu^f) \ | \ \mu^f \in \gamma_f \}$ for the reduced right-hand side in (\ref{eq:QLF_expansion}). 
% \beq
% \label{eq:Frb}
% F_{rb,\gamma} = [Q^T f_h(\mu^f_1) \ \ Q^T f_h(\mu^f_2) \ \ \dots \ \ Q^T f_h(\mu^f_{n_f})]
% \eeq
The detailed algorithm of this section can be found in Algorithm $2$.


%\textbf{Step 4 (Offline): Set up the least squares problems.}
\subsection{Least squares problems (Offline$\backslash$Online)}
% We find the coefficients $c_j^l(\mu)$ and $c_j^f(\mu)$ in (\ref{eq:LF_expansion}) and (\ref{eq:QLF_expansion}) by solving least squares problems in the online stage. 
In the online stage, the reduced operators and the right-hand sides for a new parameter $\mu$ will be approximated by the expansions (\ref{eq:QLF_expansion}). Thus, the expansion coefficients in (\ref{eq:QLF_expansion}) need to be computed. This is done by solving least-squares problems using (\ref{eq:LF_expansion}). In this section, we introduce the least-squares problem and its offline-online decomposition.  

To efficiently approximate the expansion coefficients in (\ref{eq:LF_expansion}):
\beq
\bsp
a_h(\mu) &= [a_h^{(1)}(\mu) \ \ \cdots \ \ a_h^{(n_L)}(\mu) ]^T\in \mathbb{R}^{n_L\times 1}, \\
b_h(\mu) &= [b_h^{(1)}(\mu) \ \ \cdots \ \ b_h^{(n_f)}(\mu) ]^T \in \mathbb{R}^{n_f\times 1},
\end{split}
\eeq
we consider the following matrix form corresponding to the equation (\ref{eq:LF_expansion}).
\beq
\label{eq:matrixlsq}
\bsp
\vec L_h(\mu) \approx {\mathcal L}_{h}(\gamma) a_h(\mu), \ F_h(\mu)\approx {\mathcal F}_{h}(\gamma)  b_h(\mu),
\end{split}
\eeq
where $\vec L_h(\mu) \in \mathbb{R}^{{\mathcal O}(N_{h})\times 1}$, %$a_h(\mu) = [a_h^{(1)}(\mu) \ \ \cdots \ \ a_h^{(n_L)}(\mu) ]^T\in \mathbb{R}^{n_L\times 1}$, $ b_h(\mu) = [b_h^{(1)}(\mu) \ \ \cdots \ \ b_h^{(n_f)}(\mu) ]^T \in \mathbb{R}^{n_f\times 1}$, 
and
\beq
\label{eq:HF_LF_gamma}
\begin{split}
{\mathcal L}_{h}(\gamma) &= [\vec{L}_h(\mu^L_1) \ \ \vec{L}_h(\mu^L_2) \ \ \cdots \ \ \vec{L}_h(\mu^L_{n_L})]\in\mathbb{R}^{{\mathcal O}(N_{h})\times n_L} \\
{\mathcal F}_{h}(\gamma) &= [f_h(\mu^f_1) \ \ f_h(\mu^f_2) \ \ \dots \ \ f_h(\mu^f_{n_f})]\in \mathbb{R}^{N_h\times n_L}.
\end{split}
\eeq
%We note that the matrices $L_{h,\gamma}$ and $F_{h,\gamma}$ are already computed when we assembled (\ref{eq:L_bar_rb}) and (\ref{eq:Frb}). 
Given a parameter $\mu$, we aim to compute $a_h(\mu)$ and $b_h(\mu)$ using the least squares approach. However, the least squares problem on using (\ref{eq:matrixlsq}) is very expensive as we need to access the high-fidelity operator and right-hand side: $L_h(\mu)$, $f_h(\mu)$. % and deal with the high-fidelity matrices $L_{h,\gamma}$, $F_{h,\gamma}$.
 To mitigate this issue, we solve the following low-fidelity equations to compute the coefficients $a_l(\mu)$, $b_l(\mu)$ as the surrogates of $a_h(\mu)$, $b_h(\mu)$ respectively.(\ref{eq:matrixlsq}).
\beq
\label{eq:matrixlsq_c}
\bsp
\vec{L}_l(\mu)\approx {\mathcal L}_{l}(\gamma) a_l(\mu), \ f_l(\mu)\approx {\mathcal F}_{l}(\gamma) b_l(\mu),
\end{split}
\eeq
where the low-fidelity expansion coefficients are
\beq
\bsp
a_l(\mu) &= [a_l^{(1)}(\mu) \ \ \cdots \ \ a_l^{(n_L)}(\mu) ]^T\in \mathbb{R}^{n_L\times 1},\\
b_l(\mu) &= [b_l^{(1)}(\mu) \ \ \cdots \ \ b_l^{(n_f)}(\mu) ]^T\in \mathbb{R}^{n_f\times 1},
\end{split}
\eeq
and
\beq
\label{eq:LF_LF}
\begin{split}
{\mathcal L}_{l}(\gamma) &= [\vec{L}_l(\mu^L_1)) \ \ \vec{L}_l(\mu^L_2)) \ \ \cdots \ \ \vec{L}_l(\mu^L_{n_L}))] \in \mathbb{R}^{{\mathcal O}(N_{l})\times n_L},\\
{\mathcal F}_{l}(\gamma) &= [f_l(\mu^f_1) \ \ f_l(\mu^f_2) \ \ \dots \ \ f_l(\mu^f_{n_f})]  \in \mathbb{R}^{N_l\times n_f}.
\end{split}
\eeq
We note again that ${\mathcal L}_{l}(\gamma)$ and ${\mathcal F}_{l}(\gamma)$ were already obtained at offline stage when we assembled ${\mathcal U}_{l}(\gamma)$ (\ref{eq:S}).
We solve (\ref{eq:matrixlsq_c}) for $a_l(\mu)$, $b_l(\mu)$ using least squared approaches. Specifically, we solve the following problems:

\beq
\label{eq:normal_c}
\begin{split}
G^L_{l,\gamma} a_l(\mu) &= g^L_{l,\gamma}(\mu), \\ 
G^F_{l,\gamma}  b_l(\mu) &= g^F_{l,\gamma}(\mu),
\end{split}
\eeq
where 
\beq
\label{eq:normal_d}
\begin{split}
G^L_{l,\gamma} &= {\mathcal L}_{l}(\gamma)^T {\mathcal L}_{l}(\gamma), \quad g^L_{l,\gamma}(\mu) = {\mathcal L}_{l}(\gamma)^T \vec L_l(\mu), \\ 
G^F_{l,\gamma} &= {\mathcal F}_{l}(\gamma)^T {\mathcal F}_{l}(\gamma), \quad 
 g^F_{l,\gamma}(\mu) = {\mathcal F}_{l}(\gamma)^T f_l(\mu)
\end{split}
\eeq
% In the offline stage, we pre-compute the matrices $(L_{l,\gamma}^T L_{l,\gamma})^{-1} L_{l,\gamma}^T$ and $(F_{l,\gamma}^T F_{l,\gamma})^{-1} F_{l,\gamma}^T$. 

For the least squares problem solve, we have the following offline-online decomposition.\\
{\bf Offline} Calculate the matrices $G^L_{l,\gamma} \in \mathbb{R}^{n_L\times n_L}$ and $G^F_{l,\gamma} \in \mathbb{R}^{n_f\times n_f}$; \\
{\bf Online} Compute $L_l(\mu)$ and $f_l(\mu)$ for a new parameter $\mu$ and solve the least squares problem (\ref{eq:normal_c})

The algorithm for the least-squares problem can be found in Algorithm $2$ and $3$.
The expansion coefficient vectors $a_l(\mu)$, $b_l(\mu)$ computed in this step will be used for the constructions of the reduced operators and right-hand sides in the next step. We note that the least squares problem is independent of our high-fidelity solver. Nonetheless, it still depends on  coarse solver, where we assume the operators and the right-hand sides based on coarse solver is much cheaper to assembly. 


% \subsection{Solving least squares problem (Online)}
% We first compute $L_{l}(\mu)$ and $f_{l}(\mu)$ for a given parameter $\mu$ using our coarse solver. Then we solve the least squares problems (\ref{eq:normal_c}) for $a_l(\mu)$, $b_l(\mu)$. This can be done by multiplying pre-computed matrices $(L_{l,\gamma}^T L_{l,\gamma})^{-1} L_{l,\gamma}^T$ and $(F_{l,\gamma}^T F_{l,\gamma})^{-1} F_{l,\gamma}^T$ to the vectors $L_{l,\gamma}(\mu)$ and $F_{l,\gamma}(\mu)$ respectively. The coefficient vectors $a_l(\mu)$, $b_l(\mu)$ computed in this step will be used for the constructions of the reduced operators and right-hand sides in the next step. We note that the least squares problem is independent of our high-fidelity solver as we only use the operators and the right-hand sides assembled from our coarse solver. 

\begin{remark}
Note that the coarse solution $u_l(\mu)$ can be easily computed using the coarse solver. Although the coarse model is usually not an accurate approximation to  the underlying  problem, it is still useful to guide the construction of reduced bases, operators, and right-hand sides.
\end{remark}

\subsection{Assembly and solving reduced problem (Online)}
\label{subsec:rb_prob}
Once the expansion coefficients are found, we can approximate the reduced operator $L_{rb}(\mu)$ and reduce right-hand side $f_{rb}(\mu)$ for a given parameter $\mu$ using the right-hand sides of (\ref{eq:QLF_expansion}),
\beq
\label{eq:QLF_expansion_red}
\bsp
\tilde{L}_{rb}(\mu) = \sum\limits_{j=1}^{n_L} [Q^T L_h(\mu^L_j) Q] \, a_l^{(j)}(\mu), \  % \sum\limits_{j=1}^{n_L} Q^T L_h(\mu^L_j) Q \, a_l^{(j)}(\mu),\\
\tilde{f}_{rb}(\mu) = \sum\limits_{j=1}^{n_f}  [Q^T f_h(\mu^f_j)] \, b_l^{(j)}(\mu) %\sum\limits_{j=1}^{n_f} Q^T f_h(\mu^f_j) \, b_l^{(j)}(\mu).
\end{split}
\eeq
We note that all matrices in the right-hand side of (\ref{eq:QLF_expansion_red}) have been pre-computed in the offline stage.
% \beq
% \bsp
% L_{rb,\gamma} = 
% F_{rb,\gamma} = 
% \end{split}
% \eeq
This step does not depend on the size of our full-order model and its complexity is independent of $N_h$.

Then we solve the following reduced problem to obtain the reduced coefficient $\tilde{u}_{rb}(\mu)$:
\beq
\label{eq:reduced_short}
\tilde{L}_{rb}(\mu) \tilde{u}_{rb}(\mu) = \tilde{f}_{rb}(\mu).
\eeq
Then the reconstructed reduced solution $u_r(\mu)$ defined in (\ref{eq:reconstructed}) can be approximated by $\tilde{u}_r(\mu) = Q \tilde{u}_{rb}(\mu) \in \mathbb{R}^{N_h}$.
%The detailed online algorithm can be found in Algorithm $3$.
% \textcolor{blue}{
% \begin{remark}
% For nonlinear problem, the operator in (\ref{eq:main}) depends on the solution $u(x,\mu)$. For full-order model, we handle nonlinearity by employing some iteration method, e.g., Picard iteration, Newton's method. 
% For example, for full-order model, we solve the linearized system $L_h(\mu;u_h^{s-1}(\mu)) u_h^s(\mu) = f_h(\mu)$ at each iteration step $s$.
% To construct ${\mathcal U}_{h}(\gamma)$ and ${\mathcal L}_{h}(\gamma)$, we use the solutions $u_h^S(\mu^u_i)$ and the operators $L_h(\mu^L_j;u_h^{S-1}(\mu^L_j))$ where $S$ represent the final iteration step. Note here that we assumed that the high-fidelity operator from the last iteration step at $\mu$, $L_h(\mu;u_h^{S-1}(\mu))$, can be approximated by a linear combination of the final iteration operators at selected parameters, $L_h(\mu^L_j;u_h^{S-1}(\mu^L_j))$, $j = 1,\dots n_L$.
% We construct ${\mathcal U}_{l}(\Gamma)$ and ${\mathcal L}_{l}(\Gamma)$ in the same way using the low-fidelity solutions $u_l^S(\mu^u_i)$ and the operators $L_l(\mu^L_j;u_l^{S-1}(\mu^L_j))$ from the last iteration step of the coarse problems. 
% %To construct the reduced problem, we use the final solutions, operators (stiffness matrix) at the last iteration step of our fine, coarse solvers.
% %For example, in (\ref{eq:S}), (\ref{eq:L}), and (\ref{eq:F}), we set $u_h(\mu_i) = u_h^S(\mu_i)$, $L_h(\mu_i) = L_h^S(u_h^{S-1},\mu_i)$, $f_h(\mu_i) = f_h^S(\mu_i)$ where $S$ stands for the last step of the iteration. 
% Then the reduced problem (\ref{eq:reduced_short}) is constructed via (\ref{eq:QLF_expansion_red}) and no iteration step is required in solving the reduced model. \textcolor{red}{not very clear}
% \end{remark}
% }

% \textcolor{blue}{
% \begin{remark}
% For nonlinear problem, the differential operator in (\ref{eq:main}) is replaced by the operator ${\mathcal L} (\mu;u(x,\mu))$  \textcolor{red}{RB literature https://arxiv.org/pdf/2101.05902.pdf, usually use ${\mathcal L} (u(x,\mu);\mu)$ }that depends on the solution $u(x,\mu)$ for a given parameter $\mu$ \textcolor{red}{I think this nonlinear setting should be put in the beginning of the problem setup section}. Numerically, the nonlinearity is typically handled by some iteration methods, e.g., Picard, or Newton's iteration method.  
% For example, for our high- and low-fidelity nonlinear models, the iteration methods converge to the numerical solution $u_h(\mu)$ and $u_l(\mu)$ respectively with some convergence criterion. Then correspondingly, the high- and low-fidelity operators converge to $L_h(\mu;u_h(\mu))$ and $L_l(\mu;u_l(\mu))$ throughout the iteration procedures. Our algorithm only requires the limit solutions and operators (not the entire sequence of them) from the legacy solver for nonlinear problems. 
% We use the high-fidelity converged solutions $u_h(\mu^u_i)$ and operators $L_h(\mu^L_j;u_h(\mu^L_j))$ obtained at selected parameters to construct the snapshot matrices ${\mathcal U}_{h}(\gamma)$ (\ref{eq:S_hat}) and ${\mathcal L}_{h}(\gamma)$ (\ref{eq:HF_LF_gamma}). \textcolor{red}{I am not sure I get your points} To find the coefficients $a_l(\mu)$ using (\ref{eq:matrixlsq_c}), the low-fidelity operator snapshot ${\mathcal L}_{l}(\Gamma)$ is constructed using the converged operators $L_l(\mu^L_j;u_l(\mu^L_j))$ and $\vec{L}_l(\mu)$ is defined by $\vec{L}_l(\mu;u_l(\mu))$. Then the reduced operator is constructed using (\ref{eq:QLF_expansion_red}). We
% %Note that the reduced operator $\tilde{L}_{rb}(\mu)$ is formed using t
% % We use the converged solutions $u_h(\mu^u_i)$ and the operators $L_h(\mu^L_j;u_h(\mu^L_j))$ obtained from the high-fidelity legacy solver at the selected parameters to construct the solution and operator snapshots, ${\mathcal U}_{h}(\gamma)$ and ${\mathcal L}_{h}(\gamma)$ respectively. 
% % ${\mathcal U}_{h}(\gamma)$ and ${\mathcal L}_{h}(\gamma)$.  
% % We construct ${\mathcal U}_{l}(\Gamma)$ and ${\mathcal L}_{l}(\Gamma)$ in the same way using the low-fidelity solutions $u_l^S(\mu^u_i)$ and the operators $L_l(\mu^L_j;u_l^{S-1}(\mu^L_j))$ from the last iteration step of the coarse problems. 
% %To construct the reduced problem, we use the final solutions, operators (stiffness matrix) at the last iteration step of our fine, coarse solvers.
% %For example, in (\ref{eq:S}), (\ref{eq:L}), and (\ref{eq:F}), we set $u_h(\mu_i) = u_h^S(\mu_i)$, $L_h(\mu_i) = L_h^S(u_h^{S-1},\mu_i)$, $f_h(\mu_i) = f_h^S(\mu_i)$ where $S$ stands for the last step of the iteration. 
% %Then the reduced problem (\ref{eq:reduced_short}) is constructed via (\ref{eq:QLF_expansion_red}) and no iteration step is required in solving the reduced model. 
% \end{remark}
% }

% \beq
% \label{eq:QLF_expansion}
% Q^T L_h(\mu) Q \approx \sum\limits_{j=1}^{n_l} Q^T L_h(\mu^l_j) Q \, c_l^{(j)}(\mu), \ 
% Q^T F_h(\mu) \approx \sum\limits_{j=1}^{n_f} Q^T F_h(\mu^f_j) \, c_f^{(j)}(\mu),
% \eeq


%w As we assume that the operators $L(\mu)$ slowly varies with respect to $\mu$, it is possible to assemble to following projected operators using the columns in $\tilde{{\mathcal L}}$.
% \beq
% \label{eq:L_rb}
% {\mathcal L}_{rb} = [\textrm{vec}(Q^TL_h(\mu_1)Q) \ \ \textrm{vec}(Q^TL_h(\mu_2)Q) \ \ \dots \ \ \textrm{vec}(Q^TL_h(\mu_p)Q)]
% \eeq

\RestyleAlgo{ruled}
\SetKwComment{Comment}{/* }{ */}


\begin{algorithm}
\caption{Constructing reduced basis (Offline)}\label{alg:offlineQ}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%\begin{algorithmic}
\Input{$\Gamma = \{\mu_1, \mu_2, \dots,\mu_{n_p}\}$, $N_{rb}$}
\Output{Reduced basis matrix $Q$}
\setstretch{1.35}
%\BlankLine
\tcc{Construct coarse-grid solutions ${\mathcal U}_{l}(\Gamma)$}
% \For{$\mu_i \in \Gamma$}{
% $L_l(\mu_i)$, $f_l(\mu_i)$, $u_l(\mu_i)$ $\longleftarrow$ CoarseFEMSolver$(\mu_i)$\;
% $U_{l,\Gamma}(:,i) = u_l(\mu_i)$
% }
${\mathcal U}_{l}(\Gamma)$, ${\mathcal L}_{l}(\Gamma)$, ${\mathcal F}_{l}(\Gamma)$ $\longleftarrow$ LFSolver($\Gamma$)  \;
\tcc{Perform Cholesky factorization on ${\mathcal U}_{l}(\Gamma)$}
Permutation vector $P_U$ $\longleftarrow$ Cholesky$({\mathcal U}_{l}(\Gamma))$\;
\tcc{Select $N_{rb}$ indices ${\mathcal I}_u$ of important columns of ${\mathcal U}_{l}(\Gamma)$}
%${\mathcal I}_s = P_{S_c}(\{i |R_{S_c,ii} \geq  \ep_s R_{S_c,11}\})$\;
${\mathcal I}_u = P_{U}(1:N_{rb})$, $\gamma_u = \{\mu_i \in \Gamma \ | \ i \in {\mathcal I}_u\}$\;
\tcc{Construct ${\mathcal U}_{h}(\gamma)$}
% \For{$i\in {\mathcal I}_u$}{
% $u_h(\mu_i)$ $\longleftarrow$ FineFEMSolver$(\mu_i)$\;
% }
${\mathcal U}_{h}(\gamma)$ $\longleftarrow$ HFSolver($\gamma_u$)\;
% $U_{h,\gamma}(:,j) = u_h(\mu_{i_j})$, $i_j \in {\mathcal I}_u$, $j = 1, \dots, n_u$\;
\tcc{Construct $Q$ by Gram-Schmidt orthogonalization on ${\mathcal U}_{h}(\gamma)$}
% $(U, \Sigma, V)$ $\longleftarrow$ GS$({\mathcal U}_{h}(\gamma))$\;
% $Q = U(:,1:N_{rb})$
$Q$ $\longleftarrow$ G-S$({\mathcal U}_{h}(\gamma))$\;
%\end{algorithmic}
\label{alg:alg_off1}
\end{algorithm}

\begin{algorithm}
\label{alg:alg_off2}
\caption{Constructing coarse and reduced operators, sources (Offline)}\label{alg:offlineLF}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%\begin{algorithmic}
\Input{$\Gamma = \{\mu_1, \mu_2, \dots,\mu_{n_p}\}$, $Q$, ${\mathcal L}_{l}(\Gamma)$, ${\mathcal F}_{l}(\Gamma)$, $n_L$, $n_f$}
\Output{$G^L_{l,\gamma}$, $G^F_{l,\gamma}$, ${\mathcal L}_{l}(\gamma)$, ${\mathcal F}_{l}(\gamma)$, Reduced L-basis, Reduced F-basis} 
\setstretch{1.35}
\tcc{Construct a basis of reduced operator}
Permutation vector $P_L$ $\longleftarrow$ Cholesky$({\mathcal L}_{l}(\Gamma))$\;
${\mathcal I}_L = P_L(:,1:n_L)$, $\gamma_L = \{\mu_i \in \Gamma \ | \ i\in {\mathcal I}_L\}$ \;
%${\mathcal I}_l = P_{{\mathcal L}_c}(\{i | R_{{\mathcal L}_c,ii} \geq  \ep_l R_{{\mathcal L}_c,11}\})$\;
${\mathcal L}_{l}(\gamma)$ $\longleftarrow$ ${\mathcal L}_{l}(\Gamma)$, $\gamma_L$\;
%${\mathcal L}_{h}(\gamma)$ $\longleftarrow$ HighFidelitySolver($\gamma_L$)\;
Reduced Operator basis: $\{Q^T L_h(\mu_{i}) Q \ | \ \mu_{i}\in \gamma_L \}$ $\longleftarrow$ HFSolver($\gamma_L$)\;
\tcc{Construct a basis of reduced right-hand side}
Permutation vector $P_F$ $\longleftarrow$ Cholesky$({\mathcal F}_{l}(\Gamma))$\;
${\mathcal I}_f = P_F(:,1:n_f)$, $\gamma_f = \{\mu_i \in \Gamma \ | \ i\in {\mathcal I}_f\}$\;
%${\mathcal I}_f = P_{{\mathcal F}_c}(\{i | R_{{\mathcal F}_c,ii} \geq  \ep_f R_{{\mathcal F}_c,11}\})$\;
${\mathcal F}_{l}(\gamma)$ $\longleftarrow$ ${\mathcal F}_{l}(\Gamma)$, $\gamma_f$\;
%${\mathcal F}_{h}(\gamma)$ $\longleftarrow$ HighFidelitySolver($\gamma_f$)\;
Reduced right-hand side basis: $\{Q^T f_h(\mu_{i}) \ | \ \mu_i \in \gamma_f \}$$\longleftarrow$ HFSolver($\gamma_f$)\;
\tcc{Compute Gramian matrices for the least squares problems}
$G^L_{l,\gamma}$, $G^F_{l,\gamma}$ $\longleftarrow$ ${\mathcal L}_{l}(\gamma)^T {\mathcal L}_{l}(\gamma)$, ${\mathcal F}_{l}(\gamma)^T {\mathcal F}_{l}(\gamma)$\; 
% pinv$(\tilde{\mathcal L}_c) \longleftarrow \tilde{\mathcal L}_c$\;
% pinv$(\tilde{\mathcal F}_c) \longleftarrow\tilde{\mathcal F}_c$
% $(L_{l,\gamma}^T L_{l,\gamma})^{-1} L_{l,\gamma}^T \longleftarrow L_{l,\gamma}$\;
% $(F_{l,\gamma}^T F_{l,\gamma})^{-1} F_{l,\gamma}^T \longleftarrow F_{l,\gamma}$
\end{algorithm}

%\begin{comment}
\begin{algorithm}
\label{alg:alg_on}
\caption{Construct and solve reduced problem(Online)}\label{alg:online}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{A parameter $\mu \in D$, $G^L_{l,\gamma}$, $G^F_{l,\gamma}$, ${\mathcal L}_{l}(\gamma)$, ${\mathcal F}_{l}(\gamma)$, Reduced L-basis, Reduced F-basis}
\Output{Reduced solution $u_r(\mu)$}
\setstretch{1.35}
$L_l(\mu)$, $f_l(\mu)$ $\longleftarrow$ LFSolver$(\mu)$\;
 %$\longleftarrow$ CoarseFEMSolver$(\mu)$\;
\tcc{Find expansion coefficients $a_l$, $b_l$}
$a_l$, $b_l$ $\longleftarrow$  Solve LS problem (\ref{eq:normal_c})\;
\tcc{Assembling reduced operator and right-hand side}
$\tilde{L}_{rb}(\mu)$ $\longleftarrow$ Reduced L-basis, $a_l$\;
$\tilde{f}_{rb}(\mu)$ $\longleftarrow$ Reduced F-basis, $b_l$\;
\tcc{Solving the reduced problem}
$\tilde{u}_{rb}(\mu)$ $\longleftarrow$ $\tilde{L}_{rb}(\mu) \backslash \tilde{f}_{rb}(\mu)$\;
\tcc{Reconstructing high-fidelity reduced solution} 
$\tilde{u}_r(\mu)$ $\longleftarrow$ $Q \tilde{u}_{rb}(\mu)$
\end{algorithm}
%\end{comment}


\section{Computational Cost}
In this section, we summarize the cost associated with the proposed algorithm. 
We note again that both high-fidelity and low-fidelity solvers for nonlinear problems involve iteration methods at given parameters. We denote by $S_h^{\textrm{max}}$, $S_l^{\textrm{max}}$ the maximum number of iteration steps overall considered parameters required for high-fidelity and low-fidelity solvers, respectively. 
%QR decompositon reference: bischof1991parallel
%sparse cholesky, lu decomposition (linear system, bended) https://user.it.uu.se/~maya/Courses/NLA/Lecture_Notes/Week_1/NLA_SparseDirect_2009_Psli.pdf, https://algowiki-project.org/en/Cholesky_method, https://www.stat.cmu.edu/~ryantibs/convexopt-F18/scribes/Lecture_19.pdf
%pivoted Cholescky decomp: On the low-rank approximation by the pivoted Cholesky decomposition
%G-S process: https://stackoverflow.com/questions/27986225/computational-complexity-of-gram-schmidt-orthogonalization-algorithm

Offline cost:
\begin{itemize}
    \item $n_p$ low-fidelity runs to collect the snapshot matrices. \jrp{I wonder if we are not specifying the complexity}
%    \textcolor{blue}{${\mathcal O}(n_p S^l_{\textrm{max}} W_l^2 N_l)$, where $W_l$ is the bandwidth of $L_l(\mu)$}
     %${\mathcal O}(n_p S^l_{\textrm{max}} N_l^3)$ 
    %\item Identifying important parameters ($\gamma_u$, $\gamma_L$, $\gamma_f$): ${\mathcal O}(N_l n_p^2) + {\mathcal O}(N_l n_p^2)+{\mathcal O}(n_p^2)$ 
    \item Identifying important parameters ($\gamma_u$, $\gamma_L$, $\gamma_f$) by pivoting Cholesky decomposition: ${\mathcal O}(n_p N_{rb}^2) + {\mathcal O}(n_p n_L^2)+{\mathcal O}(n_p n_f^2)$ %pivoted cholesky

    %${\mathcal O}(N_l n_p^2) + {\mathcal O}(N_l^2 n_p^2)+{\mathcal O}(n_p^2)$ 
    \item $N_{rb}+n_L+n_f$ high-fidelity runs. 
    %\textcolor{blue}{${\mathcal O}((N_{rb}+n_L+n_f) S_h^{\textrm{max}} W_h^2 N_h)$, where $W_h$ is the bandwidth of $L_h(\mu)$}
    %${\mathcal O}((N_{rb}+n_L+n_f) S_h^{\textrm{max}} N_h^3)$
    %\item Performing SVD to construct the reduced basis $Q$: ${\mathcal O}(N_h n_u^2)$ 
    \item Performing Gram-Schmidt orthogalization to construct the reduced basis $Q$ \textcolor{red}{only for high-fidelity? (\jrp{yes.})}: ${\mathcal O}(N_h N_{rb}^2)$ 
    \item Assembling reduced basis for operator, right-hand sides \textcolor{red}{only for high-fidelity?}:\\ ${\mathcal O}(n_L(N_{rb}N_h^2+N_{rb}^2 N_h))+{\mathcal O}(n_f N_{rb} N_h)$ \\
%    \textcolor{blue}{or ${\mathcal O}(n_L(N_{rb}N_h+N_{rb}^2 N_h))+{\mathcal O}(n_f N_{rb} N_h)$ for sparse matrix}(\cite{chaturantabut2010nonlinear})
%    \item Compute Gramian matrix $G^L_{\gamma}$, $G^F_{\gamma}$ for the least square problem in \eqref{eq:normal_d}: ${\mathcal O}(n_L^2 N_{l}) + {\mathcal O}(n_f^2 N_l)$ 
\end{itemize}

Online cost:
\begin{itemize}
    \item For given a new parameter $\mu$, run a low-fidelity solver to obtain $g^L_{l,\gamma}(\mu)$, $g^F_{l,\gamma}(\mu)$ (\ref{eq:normal_d}) for the least squares problem : 
    ${\mathcal O}(N_l^3) + {\mathcal O}((n_L+n_f) N_{l})$
    %The time complexity of this step is \textcolor{red}{we might still need to solve the solution?}${\mathcal O}(N_l^3) + {\mathcal O}(n_L N_{l})$.   
    \item Solving the least squares problems to the low-fidelity coefficients for  reduced operator and right-hand side in \eqref{eq:normal_c}: ${\mathcal O}(n_L^3)$
    \item Assembling reduced operators ${\mathcal O}(n_L N_{rb}^2)$ and right-hand sides ${\mathcal O}(n_f N_{rb})$ in \eqref{eq:QLF_expansion_red}.
    \item Solving the reduced system  in \eqref{eq:reduced_short}: ${\mathcal O}(N_{rb}^3)$.
\end{itemize}
Note that the offline stage is performed only once, and the major cost arises from the
$N_{rb}+n_L+n_f$ number of high fidelity simulations.

\begin{comment}
\begin{itemize}
    \item Solving for $n_p$ low-fidelity samples to collect the snapshot matrices:
    \textcolor{blue}{${\mathcal O}(n_p S^l_{\textrm{max}} W_l^2 N_l)$, where $W_l$ is the bandwidth of $L_l(\mu)$}
     %${\mathcal O}(n_p S^l_{\textrm{max}} N_l^3)$ 
    %\item Identifying important parameters ($\gamma_u$, $\gamma_L$, $\gamma_f$): ${\mathcal O}(N_l n_p^2) + {\mathcal O}(N_l n_p^2)+{\mathcal O}(n_p^2)$ 
    \item Identifying important parameters ($\gamma_u$, $\gamma_L$, $\gamma_f$): ${\mathcal O}(n_p N_{rb}^2) + {\mathcal O}(n_p n_L^2)+{\mathcal O}(n_p n_f^2)$ %pivoted cholesky

    %${\mathcal O}(N_l n_p^2) + {\mathcal O}(N_l^2 n_p^2)+{\mathcal O}(n_p^2)$ 
    \item Perform $N_{rb}+n_L+n_f$ high-fidelity samples: 
    \textcolor{blue}{${\mathcal O}((N_{rb}+n_L+n_f) S_h^{\textrm{max}} W_h^2 N_h)$, where $W_h$ is the bandwidth of $L_h(\mu)$}
    %${\mathcal O}((N_{rb}+n_L+n_f) S_h^{\textrm{max}} N_h^3)$
    %\item Performing SVD to construct the reduced basis $Q$: ${\mathcal O}(N_h n_u^2)$ 
    \item Performing Gram-Schmidt orthogalization to construct the reduced basis $Q$ \textcolor{red}{only for high-fidelity?}: ${\mathcal O}(N_h N_{rb}^2)$ 
    \item Assembling reduced basis for operator, right-hand sides \textcolor{red}{only for high-fidelity?}:\\ ${\mathcal O}(n_L(N_{rb}N_h^2+N_{rb}^2 N_h))+{\mathcal O}(n_f N_{rb} N_h)$ \\
    \textcolor{blue}{or ${\mathcal O}(n_L(N_{rb}N_h+N_{rb}^2 N_h))+{\mathcal O}(n_f N_{rb} N_h)$ for sparse matrix}(\cite{chaturantabut2010nonlinear})
    \item Compute Gramian matrix $G^L_{\gamma}$, $G^F_{\gamma}$ in \eqref{eq:normal_d}: ${\mathcal O}(n_L^2 N_{l}) + {\mathcal O}(n_f^2 N_l)$ 
\end{itemize}

Online cost:
\begin{itemize}
    \item For given a new parameter $\mu$, constructing least squares problems consists of solving a coarse problem for a given $\mu$ to compute coarse operator, assembling the right-hand side ${\mathcal L}_{l}(\gamma)^T \vec{L}_l(\mu)$. The time complexity of this step is \textcolor{red}{should not be $N_l^3$}${\mathcal O}(N_l^3) + {\mathcal O}(n_L N_{l})$.   
    \item Solving the least squares problems ${\mathcal O}(n_L^3)$ in \eqref{eq:normal_c}
    \item Assembling reduced operators ${\mathcal O}(n_L N_{rb}^2)$ and right-hand sides ${\mathcal O}(n_f N_{rb})$ in \eqref{eq:QLF_expansion_red}.
    \item Solve the reduce system ${\mathcal O}(N_{rb}^3)$ in \eqref{eq:reduced_short}.
\end{itemize}
\end{comment}
% The offline cost is dominated by solving high- and low-fidelity problems at many parameters. The computational cost of solving coarse problems at $\Gamma = \{\mu_1, \mu_2, \dots,\mu_{n_p}\}$ is ${\mathcal O}(n_p N_l^q)$, where $q\leq 3$ depends on detailed algorithms. Solving high-fidelity problems at selected parameters yields the computation cost at most ${\mathcal O}((n_u+n_L+n_f)N_h^q)$, where $q\leq 3$. 

% The offline portion of least squares problems consists of assembling $L_{l,\gamma}^T L_{l,\gamma} \in \mathbb{R}^{n_L\times n_L}$ and $F_{l,\gamma}^T F_{l,\gamma} \in \mathbb{R}^{n_f\times n_f}$ that correspond to time complexity ${\mathcal O}(n_L^2 N_l^2)$ and ${\mathcal O}(n_f^2 N_l)$ respectively.
% In the online stage, the least squares problems consist of constructing a coarse operator for a given $\mu$, assembling the right-hand side $L_{l,\gamma}^T \textrm{vec}(L_l(\mu))$, and solving the least-squares problems. The time complexity of this procedure is ${\mathcal O}(N_l^q) + {\mathcal O}(n_L N_z)+ {\mathcal O}(n_L^3)$.
% Assembling reduced operators and right-hand sides belongs to the online stage and has complexity ${\mathcal O}(n_LN_{rb}^2)$ and ${\mathcal O}(n_fN_{rb})$ respectively. Finally, solving the reduced problem has a computational cost ${\mathcal O}(N_{rb}^3)$.
% \textcolor{red}{comment out dominant cost?}


% \section{Error analysis}
% \label{sec:analysis}
% % We consider the following rank revealing QR factorization of ${\mathcal F}_l(\Gamma)$
% % \beq
% % {\mathcal F}_l(\Gamma) = 
% % \eeq
% For analysis purpose, we assume that all columns of ${\mathcal L}_l(\Gamma)$, ${\mathcal F}_l(\Gamma)$ are approximated by an expansion of columns of ${\mathcal L}_l(\gamma)$, ${\mathcal F}_l(\gamma)$ respectively. Then we have the following approximations to the matrices ${\mathcal L}_l(\Gamma)$, ${\mathcal F}_l(\Gamma)$.
% \beq
% %\bsp
% \label{eq:approxLF}
% \tilde{\mathcal L}_l(\Gamma) = {\mathcal L}_l(\gamma) A_l, \
% \tilde{\mathcal F}_l(\Gamma) = {\mathcal F}_l(\gamma) B_l,
% %\end{split}
% \eeq
% where $A_l$, $B_l$ are the expansion coefficients matrices of the respective sizes $n_L\times n_p$, $n_f\times n_p$. We note that the expansion coefficient matrices can be computed by least-squares problems following the framework of our method. In this paper, we consider the cases where the matrices ${\mathcal L}_l(\gamma)$ and ${\mathcal F}_l(\gamma)$ are of full ranks. However when the matrices are ill-conditioned, we can find the solutions $A_l$ or $B_l$ that minimizes $||A_l ||$ or $||B_l ||$, where $|| \cdot ||$ represent the matrix-induced $l_2$ norm.
% Then we have the following lemma introduced in \cite[Lemma 3.1]{martinsson2011randomized}. 
% \begin{lemma}
% We have the following properties of the above approximations (\ref{eq:approxLF}).
% \begin{enumerate}
% \item $\norm{A_l} \leq \sqrt{n_L(n_p-n_L)+1}, \ \norm{B_l} \leq \sqrt{n_f(n_p-n_f)+1}$,
% \item ${\mathcal L}_l(\Gamma) = \tilde{\mathcal L}_l(\Gamma)$ when $n_L \geq \min{(n_p, N_l^2)}$, \ 
% ${\mathcal F}_l(\Gamma) = \tilde{\mathcal F}_l(\Gamma)$ when $n_f \geq \min{(n_p, N_l)}$,
% \item $\norm{{\mathcal L}_l(\Gamma) - \tilde{\mathcal L}_l(\Gamma)} \leq \sqrt{n_L(n_p-n_L)+1} \, \sigma_{n_L+1}$ when $n_L < \min{(n_p, N_l^2)}$\\
% $\norm{{\mathcal F}_l(\Gamma) - \tilde{\mathcal F}_l(\Gamma)} \leq \sqrt{n_f(n_p-n_f)+1} \, \sigma_{n_f+1}$ when $n_f < \min{(n_p, N_l)}$,
% \end{enumerate}
% where $\norm{\cdot}$ is the matrix induced $l_2$ norm, and $\sigma_{n_L+1}$, $\sigma_{n_f+1}$ denote ($n_L+1$)th, (${n_f+1}$)th singular values of ${\mathcal L}_l(\Gamma)$, ${\mathcal F}_l(\Gamma)$ respectively.
% \end{lemma}

% Then the bi-fidelity approximations $\tilde{{\mathcal L}}_h(\Gamma)$, $\tilde{\mathcal F}_h(\Gamma)$ of high fidelity operator matrix ${\mathcal L}_h(\Gamma)$, right-hand side matrix ${\mathcal F}_h(\Gamma)$ are given by
% \beq
% %\bsp
% \tilde{\mathcal L}_h(\Gamma) = {\mathcal L}_h(\gamma) A_l, \
% \tilde{\mathcal F}_h(\Gamma) = {\mathcal F}_h(\gamma) B_l.
% %\end{split}
% \eeq
% We are interested in the upper bound of the error $\norm{{\mathcal L}_h(\Gamma) - \tilde{\mathcal L}_h(\Gamma)}$ and  $\norm{{\mathcal F}_h(\Gamma) - \tilde{\mathcal F}_h(\Gamma)}$. 
% We assume that there exist matrices $T_L  \in \mathbb{R}^{N_l^2 \times N_h^2}$, $T_F \in \mathbb{R}^{N_l \times N_h}$ such that $\norm{T_L}$, $\norm{T_F}$ are bounded and ${\mathcal L}_h(\Gamma) \approx T_L {\mathcal L}_l(\Gamma)$, ${\mathcal F}_h(\Gamma) \approx T_L {\mathcal F}_l(\Gamma)$ with errors $E_L$, $E_F$ respectively, i.e.,
% \beq
% {\mathcal L}_h(\Gamma) = T_L {\mathcal L}_l(\Gamma) + E_L, \  {\mathcal F}_h(\Gamma) = T_F {\mathcal F}_l(\Gamma) + E_F.
% \eeq
% Then we have 
% \beq
% \bsp
% \norm{{\mathcal L}_h(\Gamma) &-\tilde{\mathcal L}_h(\Gamma)} \\
% &\leq \norm{{\mathcal L}_h(\Gamma)-T_L {\mathcal L}_l(\Gamma)}+ \norm{T_L {\mathcal L}_l(\Gamma)-T_L \tilde{\mathcal L}_l(\Gamma)}
% +\norm{T_L \tilde{\mathcal L}_l(\Gamma)- \tilde{\mathcal L}_h(\Gamma)}\\
% &\leq \norm{{\mathcal L}_h(\Gamma)-T_L {\mathcal L}_l(\Gamma)}+\norm{T_L}\norm{{\mathcal L}_l(\Gamma)-\tilde{\mathcal L}_l(\Gamma)}
% + \norm{T_L {\mathcal L}_l(\gamma)- {\mathcal L}_h(\gamma)}\norm{A_l}\\
% &\leq \norm{{\mathcal L}_h(\Gamma)-T_L {\mathcal L}_l(\Gamma)}+\norm{T_L}\norm{{\mathcal L}_l(\Gamma)-\tilde{\mathcal L}_l(\Gamma)}
% + \norm{T_L {\mathcal L}_l(\Gamma)- {\mathcal L}_h(\Gamma)}\norm{A_l}\\
% &\leq (1+\norm{A_l})\norm{E_L}+\norm{T_L}\norm{{\mathcal L}_l(\Gamma)-\tilde{\mathcal L}_l(\Gamma)}
% \end{split}
% \eeq
% and similarly,
% \beq
% \norm{{\mathcal F}_h(\Gamma) -\tilde{\mathcal F}_h(\Gamma)} 
% \leq (1+\norm{B_l})\norm{E_F}+\norm{T_F}\norm{{\mathcal F}_l(\Gamma)-\tilde{\mathcal F}_l(\Gamma)}
% \eeq



==> Setupv1.tex <==

\section{Problem setup}

For ease of presentation, we consider the following time independent parametrized partial differential equations:
\beq
\label{eq:main}
{\mathcal L}(\mu) u(x,\mu) = f(x,\mu), \ \  x \in  \Omega \subset \mathbb{R}^n,
\eeq
where ${\mathcal L} (\mu) $ is the differential operator and some proper boundary conditions are given. For a given physical/uncertain parameter $\mu = (\mu_1, \mu_2, \dots, \mu_d) \in D\subset \mathbb{R}^d$, the solutions to (\ref{eq:main}) are often approximated by solving the corresponding discrete system:
\beq
\label{eq:main_discrete}
L_h(\mu) u_h(\mu) = f_h(\mu),
\eeq
where $L_h(\mu)\in \mathbb{R}^{N_h\times N_h}$ represent the discrete operator and $u_h(\mu)\in\mathbb{R}^{N_h}$ is the approximated  solution. The number $N_h$ is typically very large to provide a sufficiently accurate approximation to $u(x,\mu)$ in (\ref{eq:main}), therefore solving such a problem with a large $N_h$ is typically computationally expensive, particularly when a large number of high-fidelity solver runs are needed, such as uncertainty quantification, design and optimization and inverse problems . 

% The parameters $\mu$ are from \textcolor{red}{${\mathcal D}_\infty$}, a sample space continuous with respect to $\mu$. 
Our goal is to efficiently approximate the solutions of the partial differential equations at a given parameter $\mu$.  The traditional projection-based reduced models assume that the truth solution $u_h(\mu)$ lives in a low-dimensional  manifold, which can be approximated by a reduced approximation space with a dimension $N_{rb}$ much smaller than $N_h$. 
% The solutions at the parameters outside ${\mathcal D}$ are approximated using interpolation. We assume that every point in ${\mathcal D}_\infty$ is sufficiently close to one of the proxies in ${\mathcal D}$.
%The traditional projection-based reduced models typically
% first construct an orthogonal basis matrix $Q \in \mathbb{R}^{N_h\times N_{rb}}$ by \textcolor{red}{by POD or error indicator?}.%, where $N_{rb} \ll N_h$, whose columns form a basis for a reduced model whose solution is $u_{rb}(\mu) \in \mathbb{R}^{N_{rb}}$. 
 Then the solution $u_h(\mu)$ to (\ref{eq:main_discrete}) is approximated by the reduced solution as follows:
 \beq
 u_r(\mu) = Q u_{rb}(\mu),
 \eeq
where  $u_{rb}(\mu)\in \mathbb{R}^{N_{rb}}$ is the reduced coefficient vector and $Q \in \mathbb{R}^{N_h\times N_{rb}}$ is the reduced basis that span the reduced approximation space.
 %\textcolor{red}{something is missing here. also need to mention the challenge here for nonlinear problems and intrusiveness, which are the motivations}
By Galerkin projection on the problem (\ref{eq:main}) on the reduced approximation space, we can get the following reduced system:
\beq
\label{eq:reduced}
L_{rb}(\mu) u_{rb}(\mu) = f_{rb}(\mu),
\eeq
where  the reduced operator $L_{rb}(\mu) \in \mathbb{R}^{N_{rb}\times N_{rb}}$ and the reduced right-hand side $L_{rb}(\mu) \in \mathbb{R}^{N_{rb}\times N_{rb}}$ are given as follows:
\beq
\label{eq:reduced2-operator}
L_{rb}(\mu)  = Q^T L_h(\mu)Q, \quad f_{rb}(\mu) =Q^T f_h(\mu),
\eeq
For linear and weak nonlinear problems, the reduced system (\ref{eq:reduced}) can be solved very efficiently thanks to the reduced dimension $N_{rb} \ll N_h$ for $u_{rb}(\mu)$. 
% We note that $Q^TL_h(\mu)Q$ is in $ \mathbb{R}^{N_{rb}\times N_{rb}}$, thus computation of (\ref{eq:reduced}) is much less expansive than that of the original problem (\ref{eq:main}). 

\textcolor{blue}{ 
Nonetheless, for general nonlinear PDEs, the assembly of the reduced matrix $L_{rb}(\mu)$ at the online stage depends on the dimension of the full-order  solutions. Therefore the computational complexity of \eqref{eq:reduced} is still dependent on the dimension of the full-order model, $N_h$.  %For more efficient solve, 
To further improve the efficiency, EIM and its variants are usually needed \cite{barrault2004empirical,chaturantabut2010nonlinear}, where one often needs to  make major modifications of the source code. %to use or recover the decomposition of $L_h(\mu)$ into the sum of the matrices independent of the parameter that can be pre-computed in offline stage. 
This modification can be time-consuming and sophisticated for large-scale complex applications.}% or not possible when the source code of the full-order  model is not accessible. }

To overcome this issue, we develop a non-intrusive reduced-order model, particularly to efficiently construct the reduced operator $L_{rb}(\mu)$ during the online stage. % and the projected right-hand side $Q^T F_h(\mu)$.
We assume we only have access to the solutions, assembly matrices, and the right-hand side of our model from the existing legacy solver. 
%We have both fine and coarse solver for each problem.  
For  any given parameter $\mu \in {\mathcal D}$, we approximate the full-order model operator $L_h(\mu) \in \mathbb{R}^{N_h\times N_h}$, and righ-hand side $f_h(\mu) \in \mathbb{R}^{N_h}$ by
\beq
\label{eq:LF_expansion}
L_h(\mu) \approx \sum\limits_{j=1}^{n_L} L_h(\mu^L_j) \, a_h^{(j)}(\mu), \ 
f_h(\mu) \approx \sum\limits_{j=1}^{n_F} f_h(\mu^F_j) \, b_h^{(j)}(\mu),
\eeq
for properly chosen parameter points  $\{\mu^L_j \in {\mathcal D}, j=1, \hdots,n_L\}$ and  $\{\mu^F_j \in {\mathcal D}, j=1, \hdots,n_F\}$.  The expansion coefficients $a_h^{(j)}(\mu)$ and $b_h^{(j)}(\mu)$ are to approximate. 

In this case,  reduced operators $L_{rb}(\mu) $ and reduced right-hand side $f_{rb}(\mu) $ can be approximated as follows:
\beq
\begin{split}
\label{eq:QLF_expansion}
L_{rb}(\mu) &= Q^T L_h(\mu) Q \approx \sum\limits_{j=1}^{n_L} [Q^T L_h(\mu^L_j) Q ]\, a_h^{(j)}(\mu) := \sum\limits_{j=1}^{n_L} L_{rb}(\mu^L_j) \, a_h^{(j)}(\mu) , \\ 
f_{rb}(\mu) &=Q^T f_h(\mu) \approx \sum\limits_{j=1}^{n_F} [Q^T f_h(\mu^F_j)] \, b_h^{(j)}(\mu) := \sum\limits_{j=1}^{n_F} f_{rb}(\mu^F_j) \, b_h^{(j)}(\mu),
\end{split}
\eeq
where that the matrices $L_{rb}(\mu^L_j)$ and vectors $f_{rb}(\mu^F_j)$ are independent of the parameter $\mu$, thus can be precomputed during the offline stage. As a result, if the expansion coefficients $a_h^{(j)}(\mu)$ and $b_h^{(j)}(\mu)$ can be efficiently approximated during the online stage, the reduced system can be well assembled with reasonable computation cost. 
In \cite{etter2023coarse}, the authors suggest an efficient way to recover the expansion coefficients $a_h^{(j)}(\mu)$ of the operators based on the single fidelity solver. 
In this work, we propose a bi-fidelity framework to surrogate high-fidelity coefficients $a_h^{(j)}(\mu)$ and $b_h^{(j)}(\mu)$ to efficiently construct the reduced model.
In the next section, we shall discuss more detail about our approach to construct and solve the reduce system \eqref{eq:QLF_expansion}. %$L_{rb}(\mu)$ and the right-hand side $f_{rb}(\mu))$ via (\ref{eq:QLF_expansion}). 

% \beq
% {\mathbb L}(\mu) u_\mu(x) = f(\mu,x), \ \  x\in\Omega \subset \mathbb{R}^n,
% \eeq
% (\jrp{some connection})
% We discretize the above equations using finite element method with $n$ 
% \beq
% \bf{K}(\mu) \bf{U}(\mu) = \bf{F}(\mu),
% \eeq
% where 


\section{Two-grid reduced-based methods}
\textcolor{blue}{In reduce order modeling, directly constructing the reduced operator $L_{rb}(\mu)$ in (\ref{eq:QLF_expansion}) may require many the full-order model runs (\ref{eq:main_discrete}) with a large set of different parameters to access the high-fidelity information online. This is computationally very expansive, and we would like to reduce the total number of  full-order runs (high-fidelity runs) at the offline stage. We employ a bi-fidelity method to utilize both coarse (low-fidelity) and fine (high-fidelity) model in the offline algorithm.} %In our algorithm, we would like to replace many full-order solves with coarse solves to significantly reduce the total number of full-order simulations in the offline stage. } 


To set up the stage for the discussion later on, we assume a coarse mesh model corresponding to the full-order (fine-mesh) model (\ref{eq:main}) is available: 
\beq
\label{eq:coarse_main}
L_l(\mu) u_l(\mu) = f_l(\mu),
\eeq
where $L_l(\mu) \in \mathbb{R}^{N_l \times N_l}$, $u_l(\mu)$, $f_l(\mu) \in \mathbb{R}^{N_l}$ for $N_l \ll N_h$. The coarse mesh model can be solved much faster than the full-order model due to less number of degrees of freedom.  Although the coarse model is less accurate, %the accuracy of (\ref{eq:coarse_main}) is less than the hi-fidelity model (\ref{eq:main_discrete}) 
the low-fidelity functions $u_l(\mu)$, $L_l(\mu)$ and $f_l(\mu)$ can capture some important features of corresponding high-fidelity functions $u_h(\mu)$, $L_h(\mu)$ and $f_h(\mu)$ respectively.
%Compared to the high-fidelity model (\ref{eq:main_discrete}), the simulation of (\ref{eq:coarse_main}) is much faster but yields  

For a parameter set $\gamma = \{\mu_1, \mu_2, \dots, \mu_{j}\}$, we denote snapshot matrices of low-fidelity solutions, operators, and the right-hand sides evaluated at the points in $\gamma$ as 
\beq
\begin{split}
&{\mathcal U}_{l}(\gamma) = [u_l(\mu_1)\ \ u_l(\mu_2)\ \ \dots \ \ u_l(\mu_{j})],\\
&{\mathcal L}_{l}(\gamma) = [\vec{L}_l(\mu_1)\ \ \vec{L}_l(\mu_2)\ \ \dots \ \ \vec{L}_l(\mu_{j})], \\
&{\mathcal F}_{l}(\gamma) = [f_l(\mu_1)\ \ f_l(\mu_2) \ \ \dots \ \ f_l(\mu_{j})],
\end{split}
\eeq
where $\vec{L}$ means the vectorized operators. For example, $\vec{L}_l(\mu_i)$ is a vector of size $N_l^2 \times 1$ containing all entries of the matrix $L_l(\mu_i)\in \mathbb{R}^{N_l \times N_l}$. But in this work, we only use the nonzero entries of the matrices $L_l(\mu_i)$ to generate $\vec{L}_l(\mu_i)$ for computational efficiency as the matrix is generally very sparse. Then the dimension of the vector $\vec{L}_l(\mu_i)$ is ${\mathcal O}(N_l)$, the number of nonzero entries of $L_l(\mu_i)$ .

Similarly, the snapshot matrices for the full-order solutions can be denoted accordingly.
\beq
\begin{split}
& {\mathcal U}_{h}(\gamma) = [u_h(\mu_1)\ \ u_h(\mu_2)\ \ \dots\ \ u_h(\mu_{j})],\\
& {\mathcal L}_{h}(\gamma) = [\vec{L}_h(\mu_1)\ \ \vec{L}_h(\mu_2)\ \ \dots\ \ \vec{L}_h(\mu_{j})], \\
&{\mathcal F}_{h}(\gamma) = [f_h(\mu_1)\ \ f_h(\mu_2)\ \ \dots \ \ f_h(\mu_{j})],
\end{split}
\eeq
We note that the dimension of the vector $\vec{L}_h(\mu_i)$ is ${\mathcal O}(N_h)$.
In this work, we shall leverage both coarse and fine models to construct the reduced system efficiently
%$Q$ and the reduced operator $L_{rb}(\mu)$ and the right-hand side $f_{rb}(\mu)$. We first outline the algorithm
as follows: \\
{\bf Offline stage}:\\
\begin{enumerate}
\item Low-fidelity runs
\begin{itemize}
\item[$-$] Consider a set of parameters $\Gamma = \{\mu_1, \mu_2, \dots,\mu_{n_p}\}$ dense enough in the parameter domain $D$.
\item[$-$] Perform low-fidelity simulations at all parameters in $\Gamma$ to obtain ${\mathcal U}_{l}(\Gamma)$, ${\mathcal L}_{l}(\Gamma)$, and ${\mathcal F}_{l}(\Gamma)$. 
\item[$-$] Select important parameters from $\Gamma$ to construct $\gamma_u = \{\mu^u_1,\mu^u_2, \dots, \mu^u_{n_u}\}$, $\gamma_L = \{\mu^L_1,\mu^L_2, \dots, \mu^L_{n_L}\}$, $\gamma_f = \{\mu^f_1,\mu^f_2, \dots, \mu^f_{n_f}\}$ 
\end{itemize}
\item High-fidelity runs
\begin{itemize}

\item[$-$] Perform high-fidelity simulations at the selected parameter set in $\gamma_u$, $\gamma_L$, and $\gamma_f$ to construct ${\mathcal U}_{h}(\gamma_u)$, ${\mathcal L}_{h}(\gamma_L)$, and ${\mathcal F}_{h}(\gamma_f)$ %(The subscript of $\gamma$ will be omitted for matrix notations for simplicity, e.g., ${\mathcal U}_{h}(\gamma_u) = {\mathcal U}_{h}(\gamma)$ )
\end{itemize}
\item Reduced basis construction
\begin{itemize}
\item[$-$]% Perform singular value decomposition to build 
 Construct the reduced basis $Q$ using ${\mathcal U}_{h}(\gamma_u)$.
\item[$-$] \textcolor{red}{Compute $L_{rb}(\mu^L)$ and $f_{rb}(\mu^f)$ in \eqref{eq:QLF_expansion} for $\mu^L \in \gamma_L$, $\mu^f \in \gamma_f$}
\end{itemize}
{\bf Online stage}:
\item For a given parameter $\mu$, run the corresponding low-fidelity solver to find the expansion coefficients   $a_l(\mu)$ and $b_l(\mu)$.
%Low-fidelity least squares problems
%\begin{itemize}
%\item[$-$] Compute ${\mathcal L}_{l}(\gamma)^T {\mathcal L}_{l}(\gamma)$ and $F_{l}(\gamma)^T F_{l}(\gamma)$
%\item[$-$] Compute $\vec{L}_l(\mu)$ for given parameter $\mu$ using low-fidelity solver
%\item[$-$] Find the expansion coefficients $a_l(\mu)$ and $b_l(\mu)$ by least squares problems
%\beq
%{\mathcal L}_{l}(\gamma)^T {\mathcal L}_{l}(\gamma) a_l(\mu) = {\mathcal L}_{l}(\gamma) ^T\vec{L}_l(\mu), \  
%F_{l}(\gamma)^T F_{l}(\gamma) b_l(\mu) = F_{l}(\gamma)^T f_l(\mu).
%\eeq
%\end{itemize}
\item Construct and solve reduced problems
\begin{itemize}
\item[$-$] Assemble the reduced operators and reduced right-hand sides by \eqref{eq:QLF_expansion}
\item[$-$] Solve the reduced system \eqref{eq:reduced}.
%\beq
% \label{eq:QLF_expansion}
%L_{rb}(\mu) \approx \sum\limits_{j=1}^{n_L} L_{rb}(\mu^L_j)\, a_l^{(j)}(\mu), \ 
%f_{rb}(\mu) \approx %\sum\limits_{j=1}^{n_F} f_{rb}(\mu^F_j) \, b_l^{(j)}(\mu),
%\eeq
\end{itemize}
\end{enumerate}
The schematic description of our algorithm is presented in Figure \ref{fig:flowchart}.  We shall explain the details of each building block of the proposed method.
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/ROC_SCHEME_V2.png}
    \caption{Flowchart of the proposed reduced method.}
    \label{fig:flowchart}
\end{figure}

% \textcolor{red}{might be a good idea to list the pesduo code to demonstrate the whole algorithm}

%\subsection{Offline algorithm}
\subsection{Point Selection and Reduced basis construction (Offline)}
We first choose a candidate set of parameters $\Gamma = \{\mu_1, \mu_2, \dots,\mu_{n_p}\} \subset D$ and assume  $\Gamma$ is large enough to represent  the parameter space. %that every parameter $\mu \in D$ is sufficiently close to one of the parameters in $\Gamma$. We consider but do not compute 
We consider the following matrix in $\mathbb{R}^{N_h\times n_p}$ of full order solutions at parameters in $\Gamma$.
\beq
\label{eq:S}
{\mathcal U}_{h}(\Gamma) = [u_h(\mu_1) \ \ u_h(\mu_2) \ \ \dots \ \ u_h(\mu_{n_p})]
\eeq
%To compute allWe want to select important columns of ${\mathcal U}_{h}(\Gamma)$ that will contribute to constructing a 
To construct the projection-based  reduced basis  $Q$, one typically performs $n_p$ high-fidelity simulations to collect all solution snapshots and perform singular value decomposition (SVD) to extract the reduced basis set. However, the computation of the high-fidelity solutions $u_h(\mu_i)$ at many different parameters $\mu_i$, $i = 1,\dots, n_p$ is very expensive. To reduce the number of high-fidelity samples, we assume the coarse-model solutions can capture the main characteristics of the high-fidelity model such that %that the selected parameters $\{\mu^u_1,\mu^u_2, \dots, \mu^u_{n_u}\}$ using $U_{l,\Gamma}$ correspond to important columns in $U_{h,\Gamma}$
it can be used to guide the selection of important parameter points.  This idea is widely used in the multi-fidelity literature \cite{zhu2014computational,zhu2017multi,etter2023coarse}. We refer interested reader for more details in ?.

Specially, we    
% \beq
% \label{eq:S}
% S = [U_h(\mu_1) \ \ U_h(\mu_2) \ \ \dots \ \ U_h(\mu_p)]
% \eeq
perform the low-fidelity simulations for (\ref{eq:coarse_main}) on 
 the candidate set $\Gamma$  to collect the following $N_l\times n_p$ snapshot matrix of the coarse solutions:
\beq
\label{eq:S_c}
{\mathcal U}_{l}(\Gamma) = [u_l(\mu_1) \ \ u_l(\mu_2) \ \ \dots \ \ u_l(\mu_{n_p})] 
\eeq
To select important parameter points, we perform column-pivoting $QR$ factorization on ${\mathcal U}_{l}(\Gamma)$.
This procedure provides a permutation of the matrix ${\mathcal U}_{l}(\Gamma)$. We select the columns corresponding to $n_u$ largest diagonal entries of the matrix $R$, and choose the $n_u$ parameters associated with the selected important columns. We refer to the selected parameters as $\gamma_u = \{\mu^u_1,\mu^u_2, \dots, \mu^u_{n_u}\} \subset \Gamma$. %\textcolor{red}{can we replace the subindex s to be r so that it can be consistent with ROM literature}
%\textbf{Step 2: Construct reduced basis.}
To construct the reduced basis for the fine mesh solutions,
we run the fine-mesh solver to obtain the high-fidelity solutions (\ref{eq:main}) {\it only} for each point in $\gamma_u$. We  denote the snapshot matrix as follows:
\beq
\label{eq:S_hat}
{\mathcal U}_{h}(\gamma) = [u_h(\mu^u_1) \ \ u_h(\mu^u_2) \ \ \dots \ \ u_h(\mu^u_{n_u})],
\eeq
where ${\mathcal U}_{h}(\gamma_u)$ is   $N_h \times n_u$ and the columns represent important solutions in ${\mathcal U}_{h}(\Gamma)$. 
We then perform SVD decomposition on ${\mathcal U}_{h}(\gamma_u)$ to obtain ${\mathcal U}_{h}(\gamma_u) = U\Sigma V^T$. To construct the reduced basis set $Q$, we select the columns of the left singular vector $U$ that correspond to the first $N_{rb}$  largest 
 singular values. The detailed algorithm of this section is presented in Algorithm $1$.

\subsection{Constructing the reduced operator and right-hand side (Offline)}
{\bf Construct the reduced operator}. To select the important points for the reduced operator $L_h(\mu)$ in \eqref{eq:LF_expansion}, 
we consider the following snapshot matrix for the  fine mesh operator $L_h$ whose columns are the vectorized full operators $L_h(\mu)$ in for candidate set $\Gamma$ in the parameter space.
\beq
\label{eq:L}
{\mathcal L}_{h}(\Gamma) = [\vec{L}_h(\mu_1) \ \ \vec{L}_h(\mu_2) \ \ \dots \ \ \vec{L}_h(\mu_{n_p})]
\eeq
%We would like to find the dominant columns of 
if ${\mathcal L}_{h}(\Gamma)$ is available, we can perform colomn-pivoting QR decomposition on it to select the important columns.  However, this requires a large number of high-fidelity runs to collect the snapshot matrix. By the same argument used to select important points for $u_h(\mu)$ in the previous section, we instead construct the corresponding snapshot matrices of operators on a coarse mesh for the candidate set $\Gamma$:
\beq
\label{eq:L_c}
{\mathcal L}_{l}(\Gamma) = [\vec{L}_l(\mu_1) \ \ \vec{L}_l(\mu_2) \ \ \dots \ \ \vec{L}_l(\mu_{n_p})]
\eeq
Note that these matrices ${\mathcal L}_{l}(\Gamma)$ have already been assembled when we build the snapshot matrix ${\mathcal U}_{l}(\Gamma)$ in the previous section. 
We then apply column-pivoting QR decomposition to ${\mathcal L}_{l}(\Gamma)$. The first $n_L$ elements of the permutation vector give the most important parameters for the operator $L$. We denote the selected parameters as 
\beq
\gamma_L = \{\mu^L_1, \mu^L_2, \dots , \mu^L_{n_L} \} \subset \Gamma.
\eeq
We then perform high-fidelity simulations for each point in $\gamma_L$ to compute the corresponding high-fidelity operators $\{ L_h(\mu^L_i) \ | \ \mu^L_i \in \gamma_L\}$. Then we project them onto the reduced approximation space spanned by the solution reduced basis set $Q$ and construct the reduced basis set $\{ Q^T L_h(\mu^L_i) Q \ | \ \mu^L_i \in \gamma_L \}$ for the reduced operator in (\ref{eq:QLF_expansion}).
During the online stage, the above reduced matrices will be used in the expansion (\ref{eq:QLF_expansion}) of the reduced operator $L_{rb}(\mu)$ at the given parameter $\mu$. 

\textcolor{blue}{
\begin{remark}
Note that all fine and coarse operators can be stored in a sparse format. The actual dimensions of the operator matrices $L_h(\mu)$, $L_l(\mu)$ at each parameter $\mu$ are equal to the number of nonzero entries of them. In general, the operator matrices are extremely sparse, and the number of nonzero entries of $L_h(\mu)$, $L_l(\mu)$ are ${\mathcal O}(N_h)$, ${\mathcal O}(N_l)$ respectively. We remark that to generate the vectorized operators $\vec{L}_h(\mu)$ and $\vec{L}_l(\mu)$, we only use the nonzero entries of the operator matrices $L_h(\mu)$ and $L_l(\mu)$. Thus, the dimensions of $\vec{L}_h(\mu)$ and $\vec{L}_l(\mu)$ are ${\mathcal O}(N_h)$, ${\mathcal O}(N_l)$ respectively.
\end{remark}
}


%\textbf{Step 3 (Offline): 
{\bf Construct reduced right-hand side}.
%Similar to the point selection for the operator $L_h$,  
 To select the important points for the reduced right-hand side  in \eqref{eq:LF_expansion}, we denote  the following right-hand side snapshot matrix in $\mathbb{R}^{N_h\times n_p}$ as follows:
\beq
\label{eq:F}
{\mathcal F}_{h}(\Gamma) = [f_h(\mu_1) \ \ f_h(\mu_2) \ \ \dots \ \ f_h(\mu_{n_p})]
\eeq
Similarly, we denote the following matrix in $\mathbb{R}^{N_l\times n_p}$ of coarse right-hand sides instead of (\ref{eq:F}). 
\beq
\label{eq:Fc}
{\mathcal F}_{l}(\Gamma) = [f_l(\mu_1) \ \ f_l(\mu_2) \ \ \dots \ \ f_l(\mu_{n_p})]
\eeq

By the same argument for point selection for constructing the reduced operator, we shall select important points informed coarse mesh snapshot matrix ${\mathcal F}_{l}(\Gamma)$, which are already available as they were generated when we obtain ${\mathcal U}_{l}(\Gamma)$ using the coarse solver. We then use pivoted-column QR factorization on ${\mathcal F}_{l}(\Gamma)$ to find the corresponding $n_f$ dominant columns. Then we select the parameters corresponding to those columns and denote them by $\gamma_f =  \{\mu^f_1, \mu^f_2, \dots, \mu^f_{n_f} \} \subset \Gamma$.  
% \beq
% \label{eq:Fhhat}
% F_{h,\gamma} = [f_h(\mu^f_1) \ \ f_h(\mu^f_2) \ \ \dots \ \ f_h(\mu^f_{n_f})]
% \eeq
We compute the reduced basis $\{Q^T f_h(\mu^f) \ | \ \mu^f \in \gamma_f \}$ for the reduced right-hand side. 
% \beq
% \label{eq:Frb}
% F_{rb,\gamma} = [Q^T f_h(\mu^f_1) \ \ Q^T f_h(\mu^f_2) \ \ \dots \ \ Q^T f_h(\mu^f_{n_f})]
% \eeq
The detailed algorithm of this section can be found in Algorithm $2$.


%\textbf{Step 4 (Offline): Set up the least squares problems.}
\subsection{Least squares problems (Offline $\backslash$ Online)}
% We find the coefficients $c_j^l(\mu)$ and $c_j^f(\mu)$ in (\ref{eq:LF_expansion}) and (\ref{eq:QLF_expansion}) by solving least squares problems in the online stage. 
In the online stage, the reduced operators and the right-hand sides for a new parameter $\mu$ will be assembled in the expansions (\ref{eq:QLF_expansion}). Thus, the expansion coefficients in (\ref{eq:QLF_expansion}) need to be computed. This is done by solving least-squares problems using (\ref{eq:LF_expansion}). In this section, we introduce the least-squares problem and its offline-online decomposition.  

To efficiently approximate the expansion coefficients in (\ref{eq:LF_expansion}):
\beq
\bsp
a_h(\mu) &= [a_h^{(1)}(\mu) \ \ \cdots \ \ a_h^{(n_L)}(\mu) ]^T\in \mathbb{R}^{n_L\times 1}, \\
b_h(\mu) &= [b_h^{(1)}(\mu) \ \ \cdots \ \ b_h^{(n_f)}(\mu) ]^T \in \mathbb{R}^{n_f\times 1},
\end{split}
\eeq
we consider the following matrix form corresponding to the equation (\ref{eq:LF_expansion}).
\beq
\label{eq:matrixlsq}
\bsp
\vec L_h(\mu) \approx {\mathcal L}_{h}(\gamma) a_h(\mu), \ F_h(\mu)\approx {\mathcal F}_{h}(\gamma)  b_h(\mu),
\end{split}
\eeq
where $\vec L_h(\mu) \in \mathbb{R}^{{\mathcal O}(N_{h})\times 1}$, %$a_h(\mu) = [a_h^{(1)}(\mu) \ \ \cdots \ \ a_h^{(n_L)}(\mu) ]^T\in \mathbb{R}^{n_L\times 1}$, $ b_h(\mu) = [b_h^{(1)}(\mu) \ \ \cdots \ \ b_h^{(n_f)}(\mu) ]^T \in \mathbb{R}^{n_f\times 1}$, 
and
\beq
\label{eq:HF_LF_gamma}
\begin{split}
{\mathcal L}_{h}(\gamma) &= [\vec{L}_h(\mu^L_1) \ \ \vec{L}_h(\mu^L_2) \ \ \cdots \ \ \vec{L}_h(\mu^L_{n_L})]\in\mathbb{R}^{{\mathcal O}(N_{h})\times n_L} \\
{\mathcal F}_{h}(\gamma) &= [f_h(\mu^f_1) \ \ f_h(\mu^f_2) \ \ \dots \ \ f_h(\mu^f_{n_f})]\in \mathbb{R}^{N_h\times n_L}.
\end{split}
\eeq
%We note that the matrices $L_{h,\gamma}$ and $F_{h,\gamma}$ are already computed when we assembled (\ref{eq:L_bar_rb}) and (\ref{eq:Frb}). 
Given a parameter $\mu$, we aim to compute $a_h(\mu)$ and $b_h(\mu)$ using the least squares approach. However, the least squares problem on using (\ref{eq:matrixlsq}) is very expensive as we need to access the high-fidelity operator and right-hand side: $L_h(\mu)$, $f_h(\mu)$.% and deal with the high-fidelity matrices $L_{h,\gamma}$, $F_{h,\gamma}$.
 To mitigate this issue, we solve the following low-fidelity equations to compute the coefficients $a_l(\mu)$, $b_l(\mu)$ as the surrogates of $a_h(\mu)$, $b_h(\mu)$ respectively.(\ref{eq:matrixlsq}).
\beq
\label{eq:matrixlsq_c}
\bsp
\vec{L}_l(\mu)\approx {\mathcal L}_{l}(\gamma) a_l(\mu), \ f_l(\mu)\approx {\mathcal F}_{l}(\gamma) b_l(\mu),
\end{split}
\eeq
where the low-fidelity expansion coefficients are
\beq
\bsp
a_l(\mu) &= [a_l^{(1)}(\mu) \ \ \cdots \ \ a_l^{(n_L)}(\mu) ]^T\in \mathbb{R}^{n_L\times 1},\\
b_l(\mu) &= [b_l^{(1)}(\mu) \ \ \cdots \ \ b_l^{(n_f)}(\mu) ]^T\in \mathbb{R}^{n_f\times 1},
\end{split}
\eeq
and
\beq
\label{eq:LF_LF}
\begin{split}
{\mathcal L}_{l}(\gamma) &= [\vec{L}_l(\mu^L_1)) \ \ \vec{L}_l(\mu^L_2)) \ \ \cdots \ \ \vec{L}_l(\mu^L_{n_L}))] \in \mathbb{R}^{{\mathcal O}(N_{l})\times n_L},\\
{\mathcal F}_{l}(\gamma) &= [f_l(\mu^f_1) \ \ f_l(\mu^f_2) \ \ \dots \ \ f_l(\mu^f_{n_f})]  \in \mathbb{R}^{N_l\times n_f}.
\end{split}
\eeq
We note again that ${\mathcal L}_{l}(\gamma)$ and ${\mathcal F}_{l}(\gamma)$ were already obtained at offline stage when we assembled ${\mathcal U}_{l}(\gamma)$ (\ref{eq:S}).
We solve (\ref{eq:matrixlsq_c}) for $a_l(\mu)$, $b_l(\mu)$ using least squared approaches. Specifically, we solve the following \textcolor{red}{normal equations}:

\beq
\label{eq:normal_c}
\begin{split}
G^L_{l,\gamma} a_l(\mu) &= g^L_{l,\gamma}(\mu), \\ 
G^F_{l,\gamma}  b_l(\mu) &= g^F_{l,\gamma}(\mu),
\end{split}
\eeq
where 
\beq
\label{eq:normal_d}
\begin{split}
G^L_{l,\gamma} &= {\mathcal L}_{l}(\gamma)^T {\mathcal L}_{l}(\gamma), \quad g^L_{l,\gamma}(\mu) = {\mathcal L}_{l}(\gamma)^T \vec L_l(\mu), \\ 
G^F_{l,\gamma} &= {\mathcal F}_{l}(\gamma)^T {\mathcal F}_{l}(\gamma), \quad 
 g^F_{l,\gamma}(\mu) = {\mathcal F}_{l}(\gamma)^T f_l(\mu)
\end{split}
\eeq
% In the offline stage, we pre-compute the matrices $(L_{l,\gamma}^T L_{l,\gamma})^{-1} L_{l,\gamma}^T$ and $(F_{l,\gamma}^T F_{l,\gamma})^{-1} F_{l,\gamma}^T$. 

For the least squares problem solve, we have the following offline-online decomposition.\\
{\bf Offline} Calculate the matrices $G^L_{l,\gamma} \in \mathbb{R}^{n_L\times n_L}$ and $G^F_{l,\gamma} \in \mathbb{R}^{n_f\times n_f}$; \\
{\bf Online} Compute $L_l(\mu)$ and $f_l(\mu)$ for a new parameter $\mu$ and solve the least squares problem (\ref{eq:normal_c})

The algorithm for the least-squares problem can be found in Algorithm $2$ and $3$.
The expansion coefficient vectors $a_l(\mu)$, $b_l(\mu)$ computed in this step will be used for the constructions of the reduced operators and right-hand sides in the next step. We note that the least squares problem is independent of our high-fidelity solver. Nonetheless, it still depends on  coarse solver, where we assume the operators and the right-hand sides based on coarse solver is much cheaper to assembly. 


% \subsection{Solving least squares problem (Online)}
% We first compute $L_{l}(\mu)$ and $f_{l}(\mu)$ for a given parameter $\mu$ using our coarse solver. Then we solve the least squares problems (\ref{eq:normal_c}) for $a_l(\mu)$, $b_l(\mu)$. This can be done by multiplying pre-computed matrices $(L_{l,\gamma}^T L_{l,\gamma})^{-1} L_{l,\gamma}^T$ and $(F_{l,\gamma}^T F_{l,\gamma})^{-1} F_{l,\gamma}^T$ to the vectors $L_{l,\gamma}(\mu)$ and $F_{l,\gamma}(\mu)$ respectively. The coefficient vectors $a_l(\mu)$, $b_l(\mu)$ computed in this step will be used for the constructions of the reduced operators and right-hand sides in the next step. We note that the least squares problem is independent of our high-fidelity solver as we only use the operators and the right-hand sides assembled from our coarse solver. 

\begin{remark}
Note that the coarse solution $u_l(\mu)$ can be easily computed using the coarse solver. Although the coarse solution $u_l(\mu)$ is usually not an accurate approximation to the solution of our problem, it is suitable to use it to guide the construction of reduced bases, operators, and right-hand sides.
\end{remark}

\subsection{Assembly and solving reduced problem (Online)}
Once the expansion coefficients are found, we can approximate the reduced operator $L_{rb}(\mu)$ and reduce right-hand side $f_{rb}(\mu)$ for a given parameter $\mu$ using the right-hand sides of (\ref{eq:QLF_expansion}),
\beq
\label{eq:QLF_expansion_red}
\bsp
\tilde{L}_{rb}(\mu) = \sum\limits_{j=1}^{n_L} L_{rb}(\mu^L_j) \, a_l^{(j)}(\mu), \  % \sum\limits_{j=1}^{n_L} Q^T L_h(\mu^L_j) Q \, a_l^{(j)}(\mu),\\
\tilde{f}_{rb}(\mu) = \sum\limits_{j=1}^{n_f} f_{rb}(\mu^f_j) \, b_l^{(j)}(\mu) %\sum\limits_{j=1}^{n_f} Q^T f_h(\mu^f_j) \, b_l^{(j)}(\mu).
\end{split}
\eeq
We note that all matrices in the right-hand side of (\ref{eq:QLF_expansion_red}) have been pre-computed in the offline stage.
% \beq
% \bsp
% L_{rb,\gamma} = 
% F_{rb,\gamma} = 
% \end{split}
% \eeq
This procedure does not depend on the size of our full-order model and its complexity is independent of $N_h$.

Then we solve the following reduced problem to obtain the reduced coefficient $\tilde{u}_{rb}(\mu)$:
\beq
\label{eq:reduced_short}
\tilde{L}_{rb}(\mu) \tilde{u}_{rb}(\mu) = \tilde{f}_{rb}(\mu).
\eeq
\textcolor{red}{Then the reconstructed reduced solution $u_r(\mu)$ can be approximated by $\tilde{u}_r(\mu) \approx Q \tilde{u}_{rb}(\mu) \in \mathbb{R}^{N}$.}
%The detailed online algorithm can be found in Algorithm $3$.
\textcolor{blue}{
\begin{remark}
For nonlinear problem, the operator in (\ref{eq:main}) depends on the solution $u(x,\mu)$. For full-order model, we handle nonlinearity by employing some iteration method, e.g., Picard iteration, Newton's method. 
For example, for full-order model, we solve the linearized system $L_h(\mu;u^{s-1}(\mu)) u_h^s(\mu) = f(\mu)$ at each iteration step $s$.
To construct ${\mathcal U}_{h}(\gamma)$ and ${\mathcal L}_{h}(\gamma)$, we use the solutions $u_h^S(\mu^u_i)$ and the operators $L_h(\mu^L_j;u^{S-1}(\mu^L_j))$ where $S$ represent the final iteration step. 
We construct ${\mathcal U}_{l}(\Gamma)$ and ${\mathcal L}_{l}(\Gamma)$ in the same way using the solutions and the operators from the last iteration step of the coarse problems. 
%To construct the reduced problem, we use the final solutions, operators (stiffness matrix) at the last iteration step of our fine, coarse solvers.
%For example, in (\ref{eq:S}), (\ref{eq:L}), and (\ref{eq:F}), we set $u_h(\mu_i) = u_h^S(\mu_i)$, $L_h(\mu_i) = L_h^S(u_h^{S-1},\mu_i)$, $f_h(\mu_i) = f_h^S(\mu_i)$ where $S$ stands for the last step of the iteration. 
Then the reduced problem (\ref{eq:reduced_short}) is constructed via (\ref{eq:QLF_expansion_red}) and no iteration step is required in solving the reduced model. \textcolor{red}{not very clear}
\end{remark}
}

% \beq
% \label{eq:QLF_expansion}
% Q^T L_h(\mu) Q \approx \sum\limits_{j=1}^{n_l} Q^T L_h(\mu^l_j) Q \, c_l^{(j)}(\mu), \ 
% Q^T F_h(\mu) \approx \sum\limits_{j=1}^{n_f} Q^T F_h(\mu^f_j) \, c_f^{(j)}(\mu),
% \eeq


%w As we assume that the operators $L(\mu)$ slowly varies with respect to $\mu$, it is possible to assemble to following projected operators using the columns in $\tilde{{\mathcal L}}$.
% \beq
% \label{eq:L_rb}
% {\mathcal L}_{rb} = [\textrm{vec}(Q^TL_h(\mu_1)Q) \ \ \textrm{vec}(Q^TL_h(\mu_2)Q) \ \ \dots \ \ \textrm{vec}(Q^TL_h(\mu_p)Q)]
% \eeq

\RestyleAlgo{ruled}
\SetKwComment{Comment}{/* }{ */}


\begin{algorithm}
\caption{Constructing reduced basis (Offline)}\label{alg:offlineQ}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%\begin{algorithmic}
\Input{$\Gamma = \{\mu_1, \mu_2, \dots,\mu_{n_p}\}$, $n_u$, $N_{rb}$}
\Output{Reduced basis matrix $Q$}
\setstretch{1.35}
%\BlankLine
\tcc{Construct coarse-grid solutions ${\mathcal U}_{l}(\Gamma)$}
% \For{$\mu_i \in \Gamma$}{
% $L_l(\mu_i)$, $f_l(\mu_i)$, $u_l(\mu_i)$ $\longleftarrow$ CoarseFEMSolver$(\mu_i)$\;
% $U_{l,\Gamma}(:,i) = u_l(\mu_i)$
% }
${\mathcal U}_{l}(\Gamma)$, ${\mathcal L}_{l}(\Gamma)$, ${\mathcal F}_{l}(\Gamma)$ $\longleftarrow$ LowFidelitySolver($\Gamma$)  \;
\tcc{Perform QR factorization on ${\mathcal U}_{l}(\Gamma)$}
Permutation vector $P_U$ $\longleftarrow$ QR$({\mathcal U}_{l}(\Gamma))$\;
\tcc{Select $n_u$ indices ${\mathcal I}_u$ of important columns of ${\mathcal U}_{l}(\Gamma)$}
%${\mathcal I}_s = P_{S_c}(\{i |R_{S_c,ii} \geq  \ep_s R_{S_c,11}\})$\;
${\mathcal I}_u = P_{U}(1:n_u)$, $\gamma_u = \{\mu_i \in \Gamma \ | \ i \in {\mathcal I}_u\}$\;
\tcc{Construct ${\mathcal U}_{h}(\gamma)$}
% \For{$i\in {\mathcal I}_u$}{
% $u_h(\mu_i)$ $\longleftarrow$ FineFEMSolver$(\mu_i)$\;
% }
${\mathcal U}_{h}(\gamma)$ $\longleftarrow$ HighFidelitySolver($\gamma_u$)\;
% $U_{h,\gamma}(:,j) = u_h(\mu_{i_j})$, $i_j \in {\mathcal I}_u$, $j = 1, \dots, n_u$\;
\tcc{Construct reduced basis matrix $Q$ by SVD on ${\mathcal U}_{h}(\gamma)$}
$(U, \Sigma, V)$ $\longleftarrow$ SVD$({\mathcal U}_{h}(\gamma))$\;
$Q = U(:,1:N_{rb})$
%\end{algorithmic}
\label{alg:alg_off1}
\end{algorithm}

\begin{algorithm}
\label{alg:alg_off2}
\caption{Constructing coarse and reduced operators, sources (Offline)}\label{alg:offlineLF}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%\begin{algorithmic}
\Input{$\Gamma = \{\mu_1, \mu_2, \dots,\mu_{n_p}\}$, $Q$, ${\mathcal L}_{l}(\Gamma)$, ${\mathcal F}_{l}(\Gamma)$, $n_L$, $n_f$}
\Output{$G^L_{l,\gamma}$, $G^F_{l,\gamma}$, ${\mathcal L}_{l}(\gamma)$, ${\mathcal F}_{l}(\gamma)$, Reduced L-basis, Reduced F-basis} 
\setstretch{1.35}
\tcc{Construct a basis of reduced operator}
Permutation vector $P_L$ $\longleftarrow$ QR$({\mathcal L}_{l}(\Gamma))$\;
${\mathcal I}_L = P_L(:,1:n_L)$, $\gamma_L = \{\mu_i \in \Gamma \ | \ i\in {\mathcal I}_L\}$ \;
%${\mathcal I}_l = P_{{\mathcal L}_c}(\{i | R_{{\mathcal L}_c,ii} \geq  \ep_l R_{{\mathcal L}_c,11}\})$\;
${\mathcal L}_{l}(\gamma)$ $\longleftarrow$ ${\mathcal L}_{l}(\Gamma)$, $\gamma_L$\;
%${\mathcal L}_{h}(\gamma)$ $\longleftarrow$ HighFidelitySolver($\gamma_L$)\;
Reduced L-basis: $\{Q^T L_h(\mu_{i}) Q \ | \ \mu_{i}\in \gamma_L \}$ $\longleftarrow$ HighFidelitySolver($\gamma_L$)\;
\tcc{Construct a basis of reduced right-hand side}
Permutation vector $P_F$ $\longleftarrow$ QR$({\mathcal F}_{l}(\Gamma))$\;
${\mathcal I}_f = P_F(:,1:n_f)$, $\gamma_f = \{\mu_i \in \Gamma \ | \ i\in {\mathcal I}_f\}$\;
%${\mathcal I}_f = P_{{\mathcal F}_c}(\{i | R_{{\mathcal F}_c,ii} \geq  \ep_f R_{{\mathcal F}_c,11}\})$\;
${\mathcal F}_{l}(\gamma)$ $\longleftarrow$ ${\mathcal F}_{l}(\Gamma)$, $\gamma_f$\;
%${\mathcal F}_{h}(\gamma)$ $\longleftarrow$ HighFidelitySolver($\gamma_f$)\;
Reduced F-basis: $\{Q^T f_h(\mu_{i}) \ | \ \mu_i \in \gamma_f \}$$\longleftarrow$ HighFidelitySolver($\gamma_f$)\;
\tcc{Compute Gramian matrices for the least squares problems}
$G^L_{l,\gamma}$, $G^F_{l,\gamma}$ $\longleftarrow$ ${\mathcal L}_{l}(\gamma)^T {\mathcal L}_{l}(\gamma)$, ${\mathcal F}_{l}(\gamma)^T {\mathcal F}_{l}(\gamma)$\; 
% pinv$(\tilde{\mathcal L}_c) \longleftarrow \tilde{\mathcal L}_c$\;
% pinv$(\tilde{\mathcal F}_c) \longleftarrow\tilde{\mathcal F}_c$
% $(L_{l,\gamma}^T L_{l,\gamma})^{-1} L_{l,\gamma}^T \longleftarrow L_{l,\gamma}$\;
% $(F_{l,\gamma}^T F_{l,\gamma})^{-1} F_{l,\gamma}^T \longleftarrow F_{l,\gamma}$
\end{algorithm}

%\begin{comment}
\begin{algorithm}
\label{alg:alg_on}
\caption{Construct and solve reduced problem(Online)}\label{alg:online}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{A parameter $\mu \in D$, $G^L_{l,\gamma}$, $G^F_{l,\gamma}$, ${\mathcal L}_{l}(\gamma)$, ${\mathcal F}_{l}(\gamma)$, Reduced L-basis, Reduced F-basis}
\Output{Reduced solution $u_r(\mu)$}
\setstretch{1.35}
$L_l(\mu)$, $f_l(\mu)$ $\longleftarrow$ LowFidelitySolver$(\mu)$\;
 %$\longleftarrow$ CoarseFEMSolver$(\mu)$\;
\tcc{Find expansion coefficients $a_l$, $b_l$}
$a_l$, $b_l$ $\longleftarrow$  Solve LS problem (\ref{eq:normal_c})\;
\tcc{Assembling reduced operator and right-hand side}
$\tilde{L}_{rb}(\mu)$ $\longleftarrow$ Reduced L-basis, $a_l$\;
$\tilde{f}_{rb}(\mu)$ $\longleftarrow$ Reduced F-basis, $b_l$\;
\tcc{Solving the reduced problem}
$\tilde{u}_{rb}(\mu)$ $\longleftarrow$ $\tilde{L}_{rb}(\mu) \backslash \tilde{f}_{rb}(\mu)$\;
\tcc{Reconstructing high-fidelity reduced solution} 
$\tilde{u}_r(\mu)$ $\longleftarrow$ $Q \tilde{u}_{rb}(\mu)$
\end{algorithm}
%\end{comment}

%\textbf{Online}: \\

%\textbf{Step 4: Construct reduced operator.}
% We assume that the operator at any parameter $\mu\in D$ can be approximated by the linear combination of the columns in $\hat{O}_h$.
% \beq
% \label{eq:L_expansion}
% L_h(\mu) \approx \sum\limits_{j=1}^{n_l} L_h(\mu^o_j) \, m_{j}(\mu)
% \eeq
% By the linearity of matrix multiplications, the reduced operator for each parameter in $D$ can be assembled in the following way. 
% \beq
% L_{h}^{rb}(\mu) =  Q^TL_h(\mu)Q \approx \sum\limits_{j=1}^l Q^TL_h(\tilde{\mu}_j)Q \, m_{j}(\mu)
% \eeq
% This saves the computation time for assembling the reduced operators at each parameter $\mu_i$. We are interested in finding the coefficients $m_{ij}$ in (\ref{eq:L_expansion}) and the reduced operators $L_{h}^{rb}(\mu)$. 
% \beq
% \label{eq:L_expansion_c}
% L_c(\mu) \approx \sum\limits_{j=1}^l L_c(\tilde{\mu}_j) m^c_{j}(\mu)
% \eeq
% We then define the operators $L_h^c(\mu)$ by
% \beq
% L_h^c(\mu) = \sum\limits_{j=1}^l L_h(\tilde{\mu}_j) m^c_{j}(\mu).
% \eeq
% We then construct a reduced operator in the following way.
% \beq
% \label{eq:L_rb_c}
% L_{c}^{rb}(\mu) = Q^TL_h^c(\mu)Q =\sum\limits_{j=1}^l Q^TL_h(\tilde{\mu}_j)Q m^c_{j}(\mu)
% \eeq
% We use $L_{c}^{rb}(\mu)$ as a surrogate of $L_{h}^{rb}(\mu)$. Note that the construction of $L_{h}^{rb}(\mu)$ and $L_{c}^{rb}(\mu)$ requires finding $m_{j}(\mu)$ and $m^c_{j}(\mu)$ respectively. One way is to perform least squares regression on (\ref{eq:L_expansion}) and (\ref{eq:L_expansion_c}). Both problems can be represented as the following least squares problems. 
% \beq
% \label{eq:LS_h}
% \tilde{\mathcal L} \bfa{m}(\mu) = \textrm{vec}(L_h(\mu)),
% \eeq
% \beq
% \label{eq:LS_c}
% \tilde{\mathcal L}_c \bfa{m}^c(\mu) = \textrm{vec}(L_c(\mu)),
% \eeq
% where we solve for $\bfa{m}(\mu),\ \bfa{m}^c(\mu) \in \mathbb{R}^l$, the vectors of $m_j(\mu)$, $m^c_j(\mu)$. Thus, we save computation time by solving (\ref{eq:LS_c}) instead of (\ref{eq:LS_h}).
% \textcolor{blue}{We assume that $L_{h}^{rb}(\mu)$ and $L_{c}^{rb}(\mu)$ are close to each other. Indicate what part in online stage was precomputed.}

% \textcolor{red}{need one more step to construct the reduced solutions after constructing the reduced operator?}


\section{Complexity analysis} \jrp{todo: solving sparse linear system}
In this section, we provide complex analysis of the proposed algorithm. 
We note again that both high-fidelity and low-fidelity solvers for nonlinear problems involve iteration methods at given parameters. We denote by $S_h^{\textrm{max}}$, $S_l^{\textrm{max}}$ the maximum number of iteration steps over all considered parameters required for high-fidelity and low-fidelity solvers respectively. 
We first consider the offline procedure.
%QR decompositon reference: bischof1991parallel
%sparse cholesky, lu decomposition (linear system, bended) https://user.it.uu.se/~maya/Courses/NLA/Lecture_Notes/Week_1/NLA_SparseDirect_2009_Psli.pdf, https://algowiki-project.org/en/Cholesky_method, https://www.stat.cmu.edu/~ryantibs/convexopt-F18/scribes/Lecture_19.pdf


Offline cost:
\begin{itemize}
    \item Solving for $n_p$ low-fidelity samples to collect the snapshot matrices: ${\mathcal O}(n_p S^l_{\textrm{max}} N_l^3)$ 
    \textcolor{blue}{or ${\mathcal O}(n_p S^l_{\textrm{max}} W^2 N_l)$, where $W$ is the bandwidth of $L_l(\mu)$}
    \item Identifying important parameters ($\gamma_u$, $\gamma_L$, $\gamma_f$): ${\mathcal O}(N_l n_p^2) + {\mathcal O}(N_l n_p^2)+{\mathcal O}(n_p^2)$ 
    %${\mathcal O}(N_l n_p^2) + {\mathcal O}(N_l^2 n_p^2)+{\mathcal O}(n_p^2)$ 
    \item Perform $n_u+n_L+n_f$ high-fidelity samples: ${\mathcal O}((n_u+n_L+n_f) S_h^{\textrm{max}} N_h^3)$\\
    \textcolor{blue}{or ${\mathcal O}((n_u+n_L+n_f) S_h^{\textrm{max}} W^2 N_h)$, where $W$ is the bandwidth of $L_h(\mu)$}
    \item Performing SVD to construct the reduced basis $Q$: ${\mathcal O}(N_h n_u^2)$ 
    \item Assembling reduced basis for operator, right-hand sides:\\ ${\mathcal O}(n_L(N_{rb}N_h^2+N_{rb}^2 N_h))+{\mathcal O}(n_f N_{rb} N_h)$ \\
    \textcolor{blue}{or ${\mathcal O}(n_L(N_{rb}N_h+N_{rb}^2 N_h))+{\mathcal O}(n_f N_{rb} N_h)$ for sparse matrix}(\cite{chaturantabut2010nonlinear})
    \item Compute Gramian matrix $G^L_{\gamma}$, $G^F_{\gamma}$: ${\mathcal O}(n_L^2 N_{l}) + {\mathcal O}(n_f^2 N_l)$ 
\end{itemize}

Online cost:
\begin{itemize}
    \item For given a new parameter $\mu$, constructing least squares problems consists of solving a coarse problem for a given $\mu$ to compute coarse operator, assembling the right-hand side ${\mathcal L}_{l}(\gamma)^T \vec{L}_l(\mu)$. The time complexity of this procedure is ${\mathcal O}(N_l^3) + {\mathcal O}(n_L N_{l})$. 
    \item Solving the least squares problems ${\mathcal O}(n_L^3)$
    \item Assembling reduced operators ${\mathcal O}(n_L N_{rb}^2)$ and right-hand sides ${\mathcal O}(n_f N_{rb})$.
    \item Solve the reduce system ${\mathcal O}(N_{rb}^3)$.
\end{itemize}
% The offline cost is dominated by solving high- and low-fidelity problems at many parameters. The computational cost of solving coarse problems at $\Gamma = \{\mu_1, \mu_2, \dots,\mu_{n_p}\}$ is ${\mathcal O}(n_p N_l^q)$, where $q\leq 3$ depends on detailed algorithms. Solving high-fidelity problems at selected parameters yields the computation cost at most ${\mathcal O}((n_u+n_L+n_f)N_h^q)$, where $q\leq 3$. 

% The offline portion of least squares problems consists of assembling $L_{l,\gamma}^T L_{l,\gamma} \in \mathbb{R}^{n_L\times n_L}$ and $F_{l,\gamma}^T F_{l,\gamma} \in \mathbb{R}^{n_f\times n_f}$ that correspond to time complexity ${\mathcal O}(n_L^2 N_l^2)$ and ${\mathcal O}(n_f^2 N_l)$ respectively.
% In the online stage, the least squares problems consist of constructing a coarse operator for a given $\mu$, assembling the right-hand side $L_{l,\gamma}^T \textrm{vec}(L_l(\mu))$, and solving the least-squares problems. The time complexity of this procedure is ${\mathcal O}(N_l^q) + {\mathcal O}(n_L N_z)+ {\mathcal O}(n_L^3)$.
% Assembling reduced operators and right-hand sides belongs to the online stage and has complexity ${\mathcal O}(n_LN_{rb}^2)$ and ${\mathcal O}(n_fN_{rb})$ respectively. Finally, solving the reduced problem has a computational cost ${\mathcal O}(N_{rb}^3)$.
% \textcolor{red}{comment out dominant cost?}


\section{Error analysis}
\label{sec:analysis}
% We consider the following rank revealing QR factorization of ${\mathcal F}_l(\Gamma)$
% \beq
% {\mathcal F}_l(\Gamma) = 
% \eeq
For analysis purpose, we assume that all columns of ${\mathcal L}_l(\Gamma)$, ${\mathcal F}_l(\Gamma)$ are approximated by an expansion of columns of ${\mathcal L}_l(\gamma)$, ${\mathcal F}_l(\gamma)$ respectively. Then we have the following approximations to the matrices ${\mathcal L}_l(\Gamma)$, ${\mathcal F}_l(\Gamma)$.
\beq
%\bsp
\label{eq:approxLF}
\tilde{\mathcal L}_l(\Gamma) = {\mathcal L}_l(\gamma) A_l, \
\tilde{\mathcal F}_l(\Gamma) = {\mathcal F}_l(\gamma) B_l,
%\end{split}
\eeq
where $A_l$, $B_l$ are the expansion coefficients matrices of the respective sizes $n_L\times n_p$, $n_f\times n_p$. We note that the expansion coefficient matrices can be computed by least-squares problems following the framework of our method. In this paper, we consider the cases where the matrices ${\mathcal L}_l(\gamma)$ and ${\mathcal F}_l(\gamma)$ are of full ranks. However when the matrices are ill-conditioned, we can find the solutions $A_l$ or $B_l$ that minimizes $||A_l ||$ or $||B_l ||$, where $|| \cdot ||$ represent the matrix-induced $l_2$ norm.
Then we have the following lemma introduced in \cite[Lemma 3.1]{martinsson2011randomized}. 
\begin{lemma}
We have the following properties of the above approximations (\ref{eq:approxLF}).
\begin{enumerate}
\item $\norm{A_l} \leq \sqrt{n_L(n_p-n_L)+1}, \ \norm{B_l} \leq \sqrt{n_f(n_p-n_f)+1}$,
\item ${\mathcal L}_l(\Gamma) = \tilde{\mathcal L}_l(\Gamma)$ when $n_L \geq \min{(n_p, N_l^2)}$, \ 
${\mathcal F}_l(\Gamma) = \tilde{\mathcal F}_l(\Gamma)$ when $n_f \geq \min{(n_p, N_l)}$,
\item $\norm{{\mathcal L}_l(\Gamma) - \tilde{\mathcal L}_l(\Gamma)} \leq \sqrt{n_L(n_p-n_L)+1} \, \sigma_{n_L+1}$ when $n_L < \min{(n_p, N_l^2)}$\\
$\norm{{\mathcal F}_l(\Gamma) - \tilde{\mathcal F}_l(\Gamma)} \leq \sqrt{n_f(n_p-n_f)+1} \, \sigma_{n_f+1}$ when $n_f < \min{(n_p, N_l)}$,
\end{enumerate}
where $\norm{\cdot}$ is the matrix induced $l_2$ norm, and $\sigma_{n_L+1}$, $\sigma_{n_f+1}$ denote ($n_L+1$)th, (${n_f+1}$)th singular values of ${\mathcal L}_l(\Gamma)$, ${\mathcal F}_l(\Gamma)$ respectively.
\end{lemma}

Then the bi-fidelity approximations $\tilde{{\mathcal L}}_h(\Gamma)$, $\tilde{\mathcal F}_h(\Gamma)$ of high fidelity operator matrix ${\mathcal L}_h(\Gamma)$, right-hand side matrix ${\mathcal F}_h(\Gamma)$ are given by
\beq
%\bsp
\tilde{\mathcal L}_h(\Gamma) = {\mathcal L}_h(\gamma) A_l, \
\tilde{\mathcal F}_h(\Gamma) = {\mathcal F}_h(\gamma) B_l.
%\end{split}
\eeq
We are interested in the upper bound of the error $\norm{{\mathcal L}_h(\Gamma) - \tilde{\mathcal L}_h(\Gamma)}$ and  $\norm{{\mathcal F}_h(\Gamma) - \tilde{\mathcal F}_h(\Gamma)}$. 
We assume that there exist matrices $T_L  \in \mathbb{R}^{N_l^2 \times N_h^2}$, $T_F \in \mathbb{R}^{N_l \times N_h}$ such that $\norm{T_L}$, $\norm{T_F}$ are bounded and ${\mathcal L}_h(\Gamma) \approx T_L {\mathcal L}_l(\Gamma)$, ${\mathcal F}_h(\Gamma) \approx T_L {\mathcal F}_l(\Gamma)$ with errors $E_L$, $E_F$ respectively, i.e.,
\beq
{\mathcal L}_h(\Gamma) = T_L {\mathcal L}_l(\Gamma) + E_L, \  {\mathcal F}_h(\Gamma) = T_F {\mathcal F}_l(\Gamma) + E_F.
\eeq
Then we have 
\beq
\bsp
\norm{{\mathcal L}_h(\Gamma) &-\tilde{\mathcal L}_h(\Gamma)} \\
&\leq \norm{{\mathcal L}_h(\Gamma)-T_L {\mathcal L}_l(\Gamma)}+ \norm{T_L {\mathcal L}_l(\Gamma)-T_L \tilde{\mathcal L}_l(\Gamma)}
+\norm{T_L \tilde{\mathcal L}_l(\Gamma)- \tilde{\mathcal L}_h(\Gamma)}\\
&\leq \norm{{\mathcal L}_h(\Gamma)-T_L {\mathcal L}_l(\Gamma)}+\norm{T_L}\norm{{\mathcal L}_l(\Gamma)-\tilde{\mathcal L}_l(\Gamma)}
+ \norm{T_L {\mathcal L}_l(\gamma)- {\mathcal L}_h(\gamma)}\norm{A_l}\\
&\leq \norm{{\mathcal L}_h(\Gamma)-T_L {\mathcal L}_l(\Gamma)}+\norm{T_L}\norm{{\mathcal L}_l(\Gamma)-\tilde{\mathcal L}_l(\Gamma)}
+ \norm{T_L {\mathcal L}_l(\Gamma)- {\mathcal L}_h(\Gamma)}\norm{A_l}\\
&\leq (1+\norm{A_l})\norm{E_L}+\norm{T_L}\norm{{\mathcal L}_l(\Gamma)-\tilde{\mathcal L}_l(\Gamma)}
\end{split}
\eeq
and similarly,
\beq
\norm{{\mathcal F}_h(\Gamma) -\tilde{\mathcal F}_h(\Gamma)} 
\leq (1+\norm{B_l})\norm{E_F}+\norm{T_F}\norm{{\mathcal F}_l(\Gamma)-\tilde{\mathcal F}_l(\Gamma)}
\eeq

% \textcolor{red}{
% error contribution \\ 
% priori error analysis based Akil's paper} \textcolor{blue}{copy from my old paper as the placeholder}
% The algorithm is a straightforward extension of the bi-fidelity method
% in \cite{Akil_mulitfidelity2013, zhu2014computational}, which
% seeks to approximate the solution at arbitrary parameter location of
% $z\in I_Z$. (Note that the method
% in \cite{Akil_mulitfidelity2013, zhu2014computational} does not require
% probability.)
% For any $z\in I_Z$, we denote
% \begin{equation} \label{epsilon}
% \epsilon(z)= \left\|u^H(z)- \P[U^H; \gamma_n, u^L(z)] \right\|^H <\infty
% \end{equation}
% the error bound of the bi-fidelity approximation. The bound was
% established in Theorem 4.4 of \cite{Akil_mulitfidelity2013}.  Its detailed
% expression is difficult to summarize without invoking too many
% notations unnecessary for this paper. Interested reader should consult
% Theorem 4.4 of \cite{Akil_mulitfidelity2013}. 

% Based upon this result, we derive the following error estimate for the
% bi-fidelity average $\mu^B(\cdot)$, compared to the high-fidelity
% average $\wE[u^H; \Gamma_N]$ (which is not feasible to compute).
% \begin{theorem}
% Let $\mu^B$ be the bi-fidelity mean \eqref{mu_B} and $\mu^H$ be the high-fidelity
% mean \eqref{mu_H}.
% If the assumptions in Theorem 4.4 of \cite{Akil_mulitfidelity2013} are
% satisfied, then
% \begin{equation}
% \left\|\mu^B(\cdot) - \mu^H(\cdot) \right\|^H \leq C_w
%  \|\epsilon(z)\|_{\ell^2(\Gamma_N)},
% \end{equation}
% where $\epsilon(z)$ is defined in \eqref{epsilon} and $C_w=\|w\|_{\ell_2}$ is the 2-norm of the weight vector
% $w=(w_1,\dots, w_N)$. Furthermore, if all weights are positive, i.e.,
% $w_i>0$, $i=1,\dots, N$, then 
% \begin{equation}
% \left\|\mu^B(\cdot) - \mu^H(\cdot)\right\|^H \leq
% \max_{z\in\Gamma_N} \epsilon(z).
% \end{equation}
% \end{theorem}
% \begin{proof}
% The  linearity of the
% operator $\P$ immediately gives us
% \begin{equation*}
% \mu^B(\cdot)= \P[ U^H; \gamma_n, \mu^L] = \P\left[ U^H; \gamma_n,
% \wE[u^L; \Gamma_N] \right]
% =\wE\left[\P\left[ U^H; \gamma_n, u^L \right]; \Gamma_N\right].
% \end{equation*}
% Then,
% \begin{equation*}
% \|\mu^B-  \mu^H\|^H
% =\left\|\wE\left[\P\left[ U^H; \gamma_n, u^L \right]-u^H; \Gamma_N\right]\right\|^H = \left\|\sum_{i=1}^N w_i
% \left(\P[ U^H; \gamma_n, u^L(z_i) ] - u^H(z_i)\right)\right\|^H.
% \end{equation*}
% A straightforward use of the Cauchy-Schwarz inequality completes
% the proof.
% \end{proof}
% \section{Choice of low-fidelity models}
